Tempura: A General Cost Based Optimizer Framework for Incremental Data Processing (Extended Version)

Incremental processing is widely-adopted in many applications, ranging from incremental view maintenance, stream computing, to recently emerging progressive data warehouse and intermittent query processing. Despite many algorithms developed on this topic, none of them can produce an incremental plan that always achieves the best performance, since the optimal plan is data dependent. In this paper, we develop a novel cost-based optimizer framework, called Tempura, for optimizing incremental data processing. We propose an incremental query planning model called TIP based on the concept of time-varying relations, which can formally model incremental processing in its most general form. We give a full specification of Tempura, which can not only unify various existing techniques to generate an optimal incremental plan, but also allow the developer to add their rewrite rules. We study how to explore the plan space and search for an optimal incremental plan. We conduct a thorough experimental evaluation of Tempura in various incremental processing scenarios to show its effectiveness and efficiency.

==> architecture.tex <==
%!TEX root=main.tex

\subsection{Example}
\label{sec:example}


% Compared to previous research which studies incremental computation in isolation
% in various settings, such as view maintenance, stream computing,
% approximate/interactive query answering and so on,
% this flexibility opens up a much larger and challenging plan space
% for progressive planning to trade-off,
% the new trade-off dimensions include:
% (1) whether the query should be progressively computed,
% (2) whether to output early results, and what kind of early results to output,
% (3) how the downstream would use the early results, and
% (4) which incremental computation method to use.


%{\bf CL: It opens up a much larger plan space for progressive planning to trade-off when jointly consider different incremental computation techniques, different data characteristics and complex dependencies along time and across queries, for which cost-based optimization becomes essential for finding the optimal progressive plan.}

In this section, we use Example~\ref{ex:pipeline} to explain the problem formulation and demonstrate the planning space.
Assume the data visible at $t_1$ and $t_2$ in \textit{sales} and \textit{returns}
are those in Fig.~\ref{fig:sales} and~\ref{fig:returns}.
A traditional data warehouse would execute the pipeline at $t_2$ when data is fully collected, and deliver results as in Fig.~\ref{fig:sales-status-full}
and~\ref{fig:summary-full}.
Instead, the progressive execution paradigm we are considering in this study can start an early execution, say at $t_1$, when only partial data is available.  A main reason of this early execution is that  there are idle resources at that time, that can be utilized with a lower price.

% To elaborate the complexity of progressive query planning,
% let us consider a periodic analytics pipeline in Example~\ref{ex:pipeline}
% that mimics many TPC-DS workloads.
% In the pipeline, the upstream \textit{sales\_status} query
% computes the final revenue of all orders by consolidating the sales orders
% with the returned ones; then a downstream \textit{summary} query
% computes the gross revenue per order category.
% \textit{sales} and \textit{returns} are two large fact tables
% that continuously synchronized from the frontend transactional databases.


% \begin{example}[A simple analytics pipeline]
% \begin{alltt}
% \small
% \textit{sales_status} =
%   SELECT \textit{sales}.\textit{o_id}, \textit{category}, \textit{price}, \textit{cost}
%   FROM \textit{sales} LEFT OUTER JOIN \textit{returns}
%     ON \textit{sales}.\textit{o_id} = \textit{returns}.\textit{o_id}

% \textit{summary} =
%   SELECT \textit{category},
%     SUM(IF(\textit{cost} IS NULL, \textit{price}, -\textit{cost})) AS \textit{gross}
%   FROM \textit{sales_status}
%   GROUP BY \textit{category}
% \end{alltt}
% \label{ex:pipeline}
% \end{example}

\hl{CL: In the figure, move those captions to the subfigures.}

\begin{figure}[htb!]
\centering
\tiny
\begin{tabular}{cccc}
\subfigure[]{
  \begin{tabular}{|c|c|c|c}
  \cline{1-3}
  \textit{o\_id} & \textit{cat} & \textit{price} & \\
  \cline{1-3}
  $o_1$ & $c_1$ & $100$ & $t_1$ \\
  \cline{1-3}
  $o_2$ & $c_2$ & $150$ & $t_1$ \\
  \cline{1-3}
  $o_3$ & $c_1$ & $120$ & $t_1$ \\
  \cline{1-3}
  $o_4$ & $c_1$ & $170$ & $t_1$ \\
  \cline{1-3}
  $o_5$ & $c_2$ & $300$ & $t_2$ \\
  \cline{1-3}
  $o_6$ & $c_1$ & $150$ & $t_2$ \\
  \cline{1-3}
  $o_7$ & $c_2$ & $220$ & $t_2$ \\
  \cline{1-3}
  \end{tabular}
  \label{fig:sales}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c}
  \cline{1-2}
  \textit{o\_id} & \textit{cost} & \\
  \cline{1-2}
  $o_1$ & $10$ & $t_1$ \\
  \cline{1-2}
  $o_2$ & $20$ & $t_2$ \\
  \cline{1-2}
  $o_6$ & $15$ & $t_2$ \\
  \cline{1-2}
  \end{tabular}
  \label{fig:returns}
}
\\
\subfigure[]{
  \begin{tabular}{|c|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{price} & \textit{cost} \\
  \hline
  $o_1$ & $c_1$ & $100$ & $10$ \\
  \hline
  $o_2$ & $c_2$ & $150$ & $20$ \\
  \hline
  $o_3$ & $c_1$ & $120$ & null \\
  \hline
  $o_4$ & $c_1$ & $170$ & null \\
  \hline
  $o_5$ & $c_2$ & $300$ & null \\
  \hline
  $o_6$ & $c_1$ & $150$ & $15$ \\
  \hline
  $o_7$ & $c_2$ & $220$ & null \\
  \hline
  \end{tabular}
  \label{fig:sales-status-full}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{cat} & \textit{gross} \\
  \hline
  $c_1$ & $265$ \\
  \hline
  $c_2$ & $500$ \\
  \hline
  \end{tabular}
  \label{fig:summary-full}
}
\\
\subfigure[]{
  \begin{tabular}{|c|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{price} & \textit{cost} \\
  \hline
  $o_1$ & $c_1$ & $100$ & $10$ \\
  \hline
  $o_2$ & $c_2$ & $150$ & null \\
  \hline
  $o_3$ & $c_1$ & $120$ & null \\
  \hline
  $o_4$ & $c_1$ & $170$ & null \\
  \hline
  \end{tabular}
  \label{fig:view-t1}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{price} & \textit{cost} & \# \\
  \hline
  \cellcolor{lightgray}$o_2$ & \cellcolor{lightgray}$c_2$ & \cellcolor{lightgray}$150$ & \cellcolor{lightgray}null & \cellcolor{lightgray}$-1$ \\
  \hline
  $o_2$ & $c_2$ & $150$ & $20$ & $+1$ \\
  \hline
  $o_5$ & $c_2$ & $300$ & null & $+1$ \\
  \hline
  $o_6$ & $c_1$ & $150$ & $15$ & $+1$ \\
  \hline
  $o_7$ & $c_2$ & $220$ & null & $+1$ \\
  \hline
  \end{tabular}
  \label{fig:view-t2}
}
\\
\subfigure[]{
  \begin{tabular}{|c|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{price} & \textit{cost} \\
  \hline
  $o_1$ & $c_1$ & $100$ & $10$ \\
  \hline
  \end{tabular}
  \label{fig:stream-t1}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{price} & \textit{cost} & \# \\
  \hline
  $o_2$ & $c_2$ & $150$ & $20$ & $+1$ \\
  \hline
  $o_3$ & $c_1$ & $120$ & null & $+1$ \\
  \hline
  $o_4$ & $c_1$ & $170$ & null & $+1$ \\
  \hline
  $o_5$ & $c_2$ & $300$ & null & $+1$ \\
  \hline
  $o_6$ & $c_1$ & $150$ & $15$ & $+1$ \\
  \hline
  $o_7$ & $c_2$ & $220$ & null & $+1$ \\
  \hline
  \end{tabular}
  \label{fig:stream-t2}
}
\end{tabular}
\caption{(a)(b) Data arrival patterns of \textit{sales} and \textit{returns}, (c)(d) results of query \textit{sales\_status} and \textit{summary} at $t_2$, (e)(f) the incremental results
of \textit{sales\_status} produced by view maintenance at $t_1,t_2$, (g)(h) the incremental
results of \textit{sales\_status} produced by stream computing at $t_1,t_2$.}
\end{figure}

\begin{comment}
\begin{figure*}[thb!]
\centering
\tiny
\begin{tabular}{cc;{2pt/2pt}cc;{2pt/2pt}cc}
\multirow{6}{*}{
  \subfigure[]{
    \includegraphics[width=0.059\textwidth]{figs/plan.pdf}
  }
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|c}
  \cline{1-3}
  \textit{o\_id} & \textit{cat} & \textit{price} & \\
  \cline{1-3}
  $o_1$ & $c_1$ & $100$ & $t_1$ \\
  \cline{1-3}
  $o_2$ & $c_2$ & $150$ & $t_1$ \\
  \cline{1-3}
  $o_3$ & $c_1$ & $120$ & $t_1$ \\
  \cline{1-3}
  $o_4$ & $c_1$ & $170$ & $t_1$ \\
  \cline{1-3}
  $o_5$ & $c_2$ & $300$ & $t_2$ \\
  \cline{1-3}
  $o_6$ & $c_1$ & $150$ & $t_2$ \\
  \cline{1-3}
  $o_7$ & $c_2$ & $220$ & $t_2$ \\
  \cline{1-3}
  \end{tabular}
  \label{fig:sales}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{price} \\
  \hline
  $o_1$ & $c_1$ & $100$ \\
  \hline
  $o_2$ & $c_2$ & $150$ \\
  \hline
  $o_3$ & $c_1$ & $120$ \\
  \hline
  $o_4$ & $c_1$ & $170$ \\
  \hline
  \end{tabular}
  \label{fig:sales-t1}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{price} & \# \\
  \hline
  $o_5$ & $c_2$ & $300$ & $+1$ \\
  \hline
  $o_6$ & $c_1$ & $150$ & $+1$ \\
  \hline
  $o_7$ & $c_2$ & $220$ & $+1$ \\
  \hline
  \end{tabular}
  \label{fig:sales-t2}
}
&
&
\\
&
\subfigure[]{
  \begin{tabular}{|c|c|c}
  \cline{1-2}
  \textit{o\_id} & \textit{cost} & \\
  \cline{1-2}
  $o_1$ & $10$ & $t_1$ \\
  \cline{1-2}
  $o_2$ & $20$ & $t_2$ \\
  \cline{1-2}
  $o_6$ & $15$ & $t_2$ \\
  \cline{1-2}
  \end{tabular}
  \label{fig:returns}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{o\_id} & \textit{cost} \\
  \hline
  $o_1$ & $10$ \\
  \hline
  \end{tabular}
  \label{fig:returns-t1}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cost} & \# \\
  \hline
  $o_2$ & $20$ & $+1$ \\
  \hline
  $o_6$ & $15$ & $+1$ \\
  \hline
  \end{tabular}
  \label{fig:returns-t2}
}
&
&
\\
\hdashline[2pt/2pt]
&
\subfigure[]{
  \begin{tabular}{|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{rev} \\
  \hline
  $o_1$ & $c_1$ & $-10$ \\
  \hline
  $o_2$ & $c_2$ & $-20$ \\
  \hline
  $o_3$ & $c_1$ & $120$ \\
  \hline
  $o_4$ & $c_1$ & $170$ \\
  \hline
  $o_5$ & $c_2$ & $300$ \\
  \hline
  $o_6$ & $c_1$ & $-15$ \\
  \hline
  $o_7$ & $c_2$ & $220$ \\
  \hline
  \end{tabular}
  \label{fig:sales-status-full}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{rev} \\
  \hline
  $o_1$ & $c_1$ & $-10$ \\
  \hline
  $o_2$ & $c_2$ & $150$ \\
  \hline
  $o_3$ & $c_1$ & $120$ \\
  \hline
  $o_4$ & $c_1$ & $170$ \\
  \hline
  \end{tabular}
  \label{fig:view-t1}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{rev} & \# \\
  \hline
  \cellcolor{lightgray}$o_2$ & \cellcolor{lightgray}$c_2$ & \cellcolor{lightgray}$150$ & \cellcolor{lightgray}$-1$ \\
  \hline
  $o_2$ & $c_2$ & $-20$ & $+1$ \\
  \hline
  $o_5$ & $c_2$ & $300$ & $+1$ \\
  \hline
  $o_6$ & $c_1$ & $-15$ & $+1$ \\
  \hline
  $o_7$ & $c_2$ & $220$ & $+1$ \\
  \hline
  \end{tabular}
  \label{fig:view-t2}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{rev} \\
  \hline
  $o_1$ & $c_1$ & $-10$ \\
  \hline
  \end{tabular}
  \label{fig:stream-t1}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{rev} & \# \\
  \hline
  $o_2$ & $c_2$ & $-20$ & $+1$ \\
  \hline
  $o_3$ & $c_1$ & $120$ & $+1$ \\
  \hline
  $o_4$ & $c_1$ & $170$ & $+1$ \\
  \hline
  $o_5$ & $c_2$ & $300$ & $+1$ \\
  \hline
  $o_6$ & $c_1$ & $-15$ & $+1$ \\
  \hline
  $o_7$ & $c_2$ & $220$ & $+1$ \\
  \hline
  \end{tabular}
  \label{fig:stream-t2}
}
\\
\hdashline[2pt/2pt]
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{cat} & \textit{gross} \\
  \hline
  $c_1$ & $265$ \\
  \hline
  $c_2$ & $500$ \\
  \hline
  \end{tabular}
  \label{fig:summary-full}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{cat} & \textit{gross} \\
  \hline
  $c_1$ & $280$ \\
  \hline
  $c_2$ & $150$ \\
  \hline
  \end{tabular}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{cat} & \textit{gross} \\
  \hline
  $c_1$ & $-15$ \\
  \hline
  $c_2$ & $+350$ \\
  \hline
  \end{tabular}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{cat} & \textit{gross} \\
  \hline
  $c_1$ & $-10$ \\
  \hline
  \end{tabular}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{cat} & \textit{gross} \\
  \hline
  $c_1$ & $+275$ \\
  \hline
  $c_2$ & $+500$ \\
  \hline
  \end{tabular}
}
\\
& &
computation at $t_1$
&
computation at $t_2$
&
computation at $t_1$
&
computation at $t_2$
\\
&
batch execution
&
\multicolumn{2}{c;{2pt/2pt}}{view maintenance progressive execution}
&
\multicolumn{2}{c}{stream computing progressive execution}
\end{tabular}
\caption{(b)(e) Data arrival of \textit{sales} and \textit{returns} respectively;
(h)(m) expected \textit{sales\_status} and \textit{summary} at $t_2$;
(c)(f)(i)(n) and (d)(g)(j)(o) progressive execution of the view maintenance approach
at $t_1,t_2$ respectively;
(k)(p) and (l)(q) progressive execution of the stream computing approach at $t_1,t_2$ respectively.\kai{[This figure will be simplified as part of it is moved into Fig.~\ref{fig:tvr-basic}.]}}
\label{fig:all-tvr-ex}
\end{figure*}
\end{comment}

%A main question is how to find a cost-efficient progressive plan for the pipeline.

Progressive computation has been studied in the contexts such as view maintenance, stream computing,
mini-batch execution and so on~\cite{bag-ivm-1,bag-ivm-2,dbtoaster,cql}. The following are two commonly used incremental computation methods.

\boldstart{View maintenance approach.}  It  would treat \textit{sales\_status} and
  \textit{summary} as views, and uses incremental computation
  to keep the views always up to date with respect to the data seen so far.
  The incremental computation is done on the delta input (e.g.,
  the delta inputs at $t_2$ are the tuples available at $t_2$ in Fig.~\ref{fig:sales}~\ref{fig:returns}).
  Figures~\ref{fig:view-t1 and}~\ref{fig:view-t2} depict \textit{sales\_status}'s
  incremental outputs at $t_1$ and $t_2$, respectively,
  where $\#=+/-$ denote insertion and deletion of tuples, respectively.
  % This would generate as many early output as possible, as shown in Fig.~\ref{fig:sales-status-retract}, and thus enable early computation of \textit{summary}.
  Note that a returning record (e.g., $r_2$ at $t_2$) can arrive much later
  than its corresponding order (e.g., the shaded $o_2$ at $t_1$).
  This approach may need to retract some of the early output results,
  such as tuple $o_2$ at Fig.~\ref{fig:view-t2}. \hl{CL: explain why.}

\boldstart{Stream computing approach.} It can avoid such retraction
  during incremental computation. Specifically in the outer join of \textit{sales\_status},
  tuples in \textit{orders} that cannot join with tuples from \textit{returns} for now
  (e.g., $o_2$, $o_3$, and $o_4$) may find a join in the future, and thus will be held back at $t_1$.
  Essentially the outer join is computed as an inner join at $t_1$.
  The incremental outputs of \textit{sales\_status} are shown
  in Fig.~\ref{fig:stream-t1}~\ref{fig:stream-t2}.


In addition to these two methods, there are many other progressive-computation methods, and which of them
delivers a better performance is {\em data dependent}. In the running example, the view maintenance approach computes $9$ tuples
($5$ tuples in the outer join and $4$ tuples in the aggregate) at $t_1$,
and $10$ tuples at $t_2$. Suppose the cost per unit at $t_1$ is 0.2 (due to fewer queries), and the cost per unit at $t_2$ is 1.  Then this approach's total cost is $9 \times 0.2 + 10 \times 1 = 11.8$.  The stream computing approach computes $6$ tuples at $t_1$, and $11$ tuple at $t_2$, with a total cost of $6 \times 0.2 + 11 \times 1 = 12.2$.
% If \textit{returns} is much smaller than \textit{sales} or most data of the two tables
% are synchronized, retraction from early outputs of \textit{sales\_status} would be rare.
The latter approach is more efficient, since it can do more early computation
in the outer join, and more early outputs further enable \textit{summary}
to carry out more early computation.
On the contrary, if the retraction is often, say, returning one more order $o_4$ at $t_2$,
then the stream computing approach will outperform, as it costs $12.2$ versus the cost of the first approach ($13.8$).
The reason is that retraction wastes early computation and causes more re-computation overhead.
The decision also depends on query dependencies of the pipeline.
If \textit{sales\_status} is consumed by many downstream queries,
any retraction from \textit{sales\_status} may cause a cascade of
re-computation, which may outweigh the benefit of early computation.

\subsection{Plan-Search Space and Challenges}

\hl{CL: The following description is too long and detailed.  I suggest we write a list of bullets to make the points more clear.}


If early computation of the entire query does not pay off,
we can still progressively execute a subpart of the query.
For instance, for the left outer join in \textit{sales\_status},
we can progressively shuffle the input data once it is ingested,
without waiting for the last time.
Progressive planning needs to search the entire continuous plan space
ranging from the traditional batch plan at one end,
to a fully-incrementalized plan at the other end.
% Actually, if early computation does not pay off, we can declare the query pipeline
% as not suitable for progressive execution, and fall back to the traditional batch plan,
% which is an extreme case in the progressive execution spectrum.

Complex dependencies can also impact the plan decision.
A small change in a dependent query can lead to very different plans.
For instance, if a \texttt{MAX} aggregate is applied on \textit{sales\_status},
retraction from \textit{sales\_status} and thus the view maintenance approach
are no longer allowed, since retraction can cause \texttt{MAX} to recompute from scratch.
The temporal aspect can further complicate the planning.
% If most returns are within two days of their sale time,
% outer joining \textit{returns} with \textit{sales} at two day earlier
% can significantly reducing the retraction.
As more and more data get ingested, the optimal physical implementation of
the outer join in \textit{sales\_status} may also change.
For instance, we may prefer a broadcast join at the beginning
when the \textit{returns} table is small.
We may change to a shuffled hash join as more data gets ingested into \textit{returns},
and change to a shuffled sort-merge join to relieve the memory pressure when \textit{returns}
gets even bigger.
However, these physical implementation decisions cannot be made in isolation
due to the dependencies between these consecutive joins in time.
Each incremental join needs to access previous data,
but shuffled hash join needs data to be distributed according to a key,
which broadcast join does not provide.
Similarly a sort-merge join requires a collation order of the data
which hash join does not satisfy.
Whether we should switch to a new join implementation
or stick to the previous implementation to avoid the above overhead
is a cost-based trade-off.

Such complex reasoning is really challenging, if not impossible,
even for the very experienced experts.
To solve this problem, we offer a cost-based solution to systematically
search the entire plan space, which can generate an efficient plans.  Our solution can
combine and exploit different incremental computation techniques in a single plan,
and have access to automatic derivations of necessary statistics.

% \subsection{Why it is non-trivial?}

% \kai{A motivating example. We can use TPC-DS queries and some user-defined changes,
% similar to the Quickr paper.}


==> discussion.tex <==
%!TEX root=main.tex

\section{Discussions}
\label{sec:discussion}

In this section, we discuss several issues incremental query planning
may encounter in practice.

\boldstart{Inaccurate data statistics.}
Data statistics is very important to cost estimation
in query optimization.
However, most incremental processing scenarios
require optimizing an incremental plan for the future,
where it is very hard to acquire accurate data statistics.
However, inaccurate statistics is not a new problem
to query optimization.
Actually, many techniques have been proposed by previous
research~\cite{robust-planning-survey}.
We believe that techniques like robust planning~\cite{graefe-robust,babu-proactive}
and parametric planning~\cite{ioannidis-parametric} can be adopted to incremental planning too.
However, it is out of the scope of this paper and we leave it to future research.
Also, we can always reoptimize the plan once we find the data
statistics is way off the previous estimation.

\boldstart{Re-optimization of incremental plans.}
An incremental plan is usually subject to change,
due to changes in the schedule of incremental processing changes,
or data statistics.
% A proposed schedule can be tentative and subject to change whenever the environment
% (such as the cluster resource usage) changes.
In this case, the original incremental plan may be only half way executed,
and have already generated and saved some intermediate states.
Blindly redoing incremental planning from scratch can waste
the saved intermediate states.
Instead, during re-planning, we can treat the saved states as materialized views,
and provide them to the optimizer for a joint consideration of the
half-way finished iterations and the new one.


% \boldstart{Workload selection for a schedule}.
% A full job pipeline can contain many queries.
% Taking the entire pipeline as a single workload for progressive planning
% may lead to an excessively large plan space, and may be too rigid for a tentative schedule.
% This problem can be avoided by planning a big workload piece-wise.
% Specifically, we can divide a big workload $W$
% into a sequence of smaller disjoint workloads $[W_1,\ldots,W_k]$,
% where $W_i \cap W_j = \emptyset$. These $W_i$'s are topologically ordered
% according to their dependency relation, i.e., $W_{i+1}$ takes the outputs of $\{W_1,\ldots,W_i\}$ as its input. We plan each $W_i$ separately in order.
% To make sure the progressive plan of $W_i$ is compatible with those of its downstream queries,
% we can include the queries dependent on $W_i$ up to a few steps, denoted $N(W_i)$.
% We can plan $W_i$ and $N(W_i)$ jointly, and only retain the physical plan
% corresponding to $W_i$ in the end.

% \S\ref{sec:single-opt} discussed optimization for a single query.
% However, as shown in \S\ref{sec:example}, in a query pipeline downstream queries
% will affect the plan choice of upstream queries.
% Thus, optimizing a single query in isolation may end up in sub-optimal progressive
% execution plans.
% To avoid stuck in local optimum, we leverage the above MQO technique for the optimization
% in query pipelines.
% Specifically, consider a pipeline where query $Q_1$ has a downstream dependent query $Q_2$.
% To optimize $Q_1$, we merge $Q_1$ and $Q_2$ into a larger query $Q_2'$,
% and jointly optimize $Q_1, Q_2'$ as a MQO problem.
% In this way, the plan choice of $Q_2'$ can indirectly affect the plan choice of $Q_1$
% through the process of picking shareable candidates.
% Note that when optimizing $Q_2'$, we add a dummy \op{QueryBoundary}
% operator to prevent $Q_2$'s operators from being pushed into $Q_1$,
% polluting the plan space of $Q_1$.
% We can generalize this process by considering queries further downstream.
% But our experimental study shows that combining the immediate downstream queries
% will already generate close-to-optimal query plans.


==> intro-chen.tex <==
%!TEX root=main.tex

\section{Introduction (CHEN; NOT USED)}
\label{sec:intro-new}

Incremental processing is a widely-used computation model
in data processing, where the input data to a query is available
progressively, and the computation of the query is triggered
multiple times  to process a delta of the input data.
With the advancement in big data systems,
both data ingestion latency and people's expectation of query latency become increasingly real time,
which further boost the application and adoption
of the incremental processing model.  As an example,
  Alibaba has warehouses of large amounts of
  automated routine data analysis, which usually have a stringent
  schedule and deadline determined by various business logic,
  e.g., scheduling a daily report query after 12 am when the previous
  day's data is fully collected and delivering the results by 6 am sharp before the bill-settlement time.
  By now, the automated routine analysis is still predominately handled using batch query processing, causing dreadful ``rush
  hour'' scheduling patterns of routine analysis jobs.
  This puts pressure on resources during traffic hours,
  and leaves the resource over-provisioned and wasted off the traffic
  hours.   Fig.~\ref{fig:resource-skew} shows the resource skew of a typical day at a company.
  Incremental processing can process routine analysis queries  progressively as data ingested,
  which have a more flexible resource usage pattern and can smooth potential resource skew. Such a problem
  also exists in many other data-centric enterprises~\cite{TOFILL}. \hl{CL: Add a citation if possible.} One effective way to
  solve this problem is to incrementally compute the answers to a query as data becomes available in the system.  For instance,
  we can run the query at several times of the day, such as 6 am, noon, 6 pm, and midnight, and use the data available at each time
  to compute the intermediate results.  In this way, we can not only reduce the latency for computing the final results, but also
  better utilize the cluster resources earlier they are more available and cheaper.

\begin{figure}[htb!]
\includegraphics[width=0.48\textwidth]{figs/resource-skew.pdf}
\caption{Cluster resource skew of a typical day at Alibaba.  The cluster tends to be very demanded, but becomes relative under utilized later in the day.}
\Description{Cluster resource skew of a typical day.}
\label{fig:resource-skew}
\end{figure}

\hl{CL: Writing flow --- (1) Different requirements; (2) Different algorithms; (3) Use an example to show that for a given query, which algorithm gives the best performance is data dependent.  (4) Problem: how to develop a solution such that given a query, it can compute the most efficient physical plan to meet the application requirement?  (5) A simple solution: run all these algorithms one by one, and choose the best one.  (6) Limitations: multiple optimization algorithms in one system, hard to implement and maintain; and not extensible to handle new incremental-computing rules. (7) Give an overview of BeanStalk and show a list of contributions.}

In general, applications that require incremental computation include~\cite{CL: add citations}.  These applications have various requirements from users on the incrementally computed results at those specified times.  For instance, some applications require {\em incremental view maintenance (IVM)}~\cite{}, which means that the intermediate results at each time should be fully computed \hl{CL: give a reason}.  \hl{CL: describe the requirement of stream processing and give a reason}.  As one more example, in the aforementioned example at Alibaba, we could want to minimize the latency of computing the final results.

Many algorithms have been developed to support incremental computation to meet application-specific requirements.  \hl{CL: mention a few algorithms and describe their main ideas.} {\bf They focus on different aspects of the problem, e.g., incremental computation methods for
a specific setting~\cite{cql,dbtoaster,outerjoin-view}, or algorithms to determine which states to materialize given
an incremental plan~\cite{intermittent}.}





% The rich research work remains isolated, and any adoption
% of incremental computation cannot leverage them
% and evolve based on that.
However, as we will show in the following example,
planning an incremental plan is more challenging than
the traditional query planning.



%
%Here, we describe a few representative emerging applications:
%
%\begin{itemize}
%  \item \textbf{Progressive Data Warehouse}.
%
%  \item \textbf{Data Cleaning}~\cite{intermittent}.
%  When querying dirty data, data usually
%  is first cleaned by a data cleaning system and then fed into the
%  database. The data cleaning system can quickly spill the clean part
%  of the data but need to conduct a time-consuming cleaning
%  processing on the dirty part. Therefore, the database can use
%  incremental processing to quickly deliver a informative but partial
%  results on the clean data to the user, before delivering the full
%  results after processing all the cleaned data.
%\end{itemize}
%



% The solution we propose is a full-fledged data warehouse solution
% based on a new execution paradigm---\emph{progressive execution}.
% The key idea is that, instead of letting all queries wait until
% their registered scheduling time, when all their input data are ready,
% whenever the data warehouse finds that the cluster has free resources,
% it can choose queries part of whose input data are ready to execute earlier,
% in order to utilize the resource.
% The early execution consumes the existing input data and saves necessary state
% for future processing of the up-coming input data, which essentially moves
% part of the computation work required off the traffic hour of the cluster,
% to a less congested time, and reduces the delivery latency of the query answer;
% it also optionally generates early outputs (not necessarily the query results),
% which in turns unblocks the downstream queries depending on it,
% so that the data warehouse can choose to early execute them later.
% Furthermore, the data warehouse can always kill an early execution
% when it sees urgent resource requirement, as the early execution is anyway speculative.
% In short, the progressive execution enable engines to execute a query at any time
% on any subset of the input data,
% and to pause and pick up the dropped-off work as wanted at any time.
% Clearly, this execution paradigm dovetails the merits of both batch and
% streaming processing paradigms:
% (1) similar to streaming computing, it enables more timely processing of accumulated
% input data and reduces the query latency,
% (2) it still processes data in a batch way during early execution with high throughput,
% but without holding resources unnecessarily,
% (3) it allows much flexible scheduling, and enables peak loads shifting,
% significantly optimizes the resource utilization of the cluster.
% \kai{[From users' perspective, better resource utilization means less resource provision
% for their analysis jobs, which leads to lower risks for missing deadlines,
% and lower resource bills.]}

% To depict the progressive execution paradigm, consider the following example
% OLAP pipeline consists of a data integration job (\texttt{ext\_sales})
% followed by an aggregation analysis (\texttt{summary}).
% \begin{example}
% \begin{alltt}
%     \small
%    ext_sales =
%     SELECT order_no, store_no, total, discount
%     FROM sales LEFT OUTER JOIN promotions
%          ON sales.promo_no=promotions.promo_no

%    summary =
%     SELECT store_no,
%       SUM(IF(discount is NULL, total, total*discount))
%     FROM ext_sales
%     GROUP BY store_no
% \end{alltt}
% \label{ex:running}
% \end{example}
% \begin{figure}[htb!]
% \centering
% \includegraphics[width=0.45\textwidth]{figs/timeline.png}
% \caption{How Example~\ref{ex:running} executes in traditional data warehouses vs \sys}
% \label{fig:timeline}
% \end{figure}
% Fig.~\ref{fig:timeline} compares how Example~\ref{ex:running} are executed
% in a traditional data warehouse and in our data warehouse \sys~on a timeline.
% Traditionally, even the data of \texttt{sales}
% and \texttt{promotions} are constantly ingested into the data warehouse
% and most is available way before the scheduled job time (at $12$am of day$2$),
% the system cannot execute \texttt{ext\_sales} and \texttt{summary},
% even though the cluster has available capacities.
% Differently \sys~can start executing \texttt{ext\_sales}
% when part of \texttt{sales} and \texttt{promotions} are available,
% and the cluster has available capacities (at $6$am, $12$pm and $18$pm of day$1$).
% Each execution can resume from the work left by the previous execution,
% and the final execution at $12$am of day$2$ finishes much faster.
% Furthermore, the early outputs of \texttt{ext\_sales} in turn
% enables the \texttt{aggregation} query to execute early too.
% Although progressive execution seems similar to traditional
% incremental computation such as view maintenance and stream computing,
% key questions in progressive execution, such as
% finding the cost-optimal progressive query plans and deciding
% when to run what queries, have significant complexity and challenges
% that are not tackled in previous research.
% This opens up a whole new line of research, and
% requires us to rethink the techniques of data warehouses,
% from query optimization to job scheduling and resource management.

% \begin{figure}[htb!]
% \centering
% \includegraphics[width=0.5\textwidth]{figs/paradigm-comparison.jpg}
% \caption{Comparison of progressive computation, stream computation and batch computation}
% \label{fig:pattern-comparison}
% \end{figure}

\eat{
Astute readers may think, ``isn't this just another form of incremental computation?''
The answer is ``yes''. Indeed, there is a rich body of research work
on various forms of incremental computation, ranging from incremental view maintenance (IVM), stream computing, to approximate/interactive query answering and so on.
However, previously these incremental techniques are
mostly studied in isolation. But as we will show below, it is a nontrivial problem
to figure out the optimal progressive execution plan exploiting these techniques.
Rather than proposing yet another incremental computation technique,
we are focusing on a unified cost-based query optimization framework
that can allow users to express and integrate various incremental computation techniques
and provide turn-key solution to decide the optimal progressive execution plans
subject to various objectives.
}

% Astute readers may think, ``isn't this just another form of incremental view maintenance (IVM)?''
% % A straightforward solution would be to adopt a small-batched solution:
% That is, one can treat a routine analysis query as a view to maintain.
% The ingested data is just updates to base relations
% % accumulated up to certain batch size or time interval,
% and triggers refresh on the view using incremental computation.
% % In this way, we do not need to wait until the scheduled time to compute
% % the analysis, but scatter the computation across the day,
% % alleviating the resource pressure on the traffic hour.
% However, this is only partially right.
% The core of progressive processing does rely on incremental computation techniques,
% but planning progressive processing is not as trivial as it looks like.
% % Progressive execution paradigm greatly extends the traditional
% % batch and streaming computation paradigms.
% % The key difference is that progressive execution can flexibly
% % schedule early execution of queries on any partial input data at any time.
% % Fig.~\ref{fig:pattern-comparison} depicts the execution patterns of the three execution paradigms.

To elaborate the complexity of incremental query planning,
let us consider incremental processing a daily analysis job
(Example~\ref{ex:pipeline}) in a progressive data warehouse.
% that consolidates sales orders with the returned ones,
% and computes the gross revenue.
% In the pipeline, the upstream \textit{sales\_status} query
% computes the final revenue of all orders by consolidating the sales orders
% with the returned ones; then a downstream \textit{summary} query
% computes the gross revenue per order category.
A progressive data warehouse may schedule early execution
of the query when only part
of tables \textit{sales} and \textit{returns} are available
but the cluster has free cheaper resources,
and thus wants to find the incremental plan with
the optimal resource usage pattern, i.e.,
carrying out as much computation as possible
in the early run to keep the overall resource bill low.
% Since tables \textit{sales} and \textit{returns} are continuously
% ingested,
% from the external transactional data sources
% the data warehouse can execute the job early before
% the schedule time
% when part of the data is already available and the cluster has
% free resources.
\begin{example}[Reporting the consolidated gross revenue]
\begin{alltt}
\footnotesize
\textit{summary} =
  with \textit{sales_status} as (
    SELECT \textit{sales}.\textit{o_id}, \textit{category}, \textit{price}, \textit{cost}
    FROM \textit{sales} LEFT OUTER JOIN \textit{returns}
      ON \textit{sales}.\textit{o_id} = \textit{returns}.\textit{o_id}
  )
  SELECT \textit{category},
    SUM(IF(\textit{cost} IS NULL, \textit{price}, -\textit{cost})) AS \textit{gross}
  FROM \textit{sales_status}
  GROUP BY \textit{category}
\end{alltt}
\label{ex:pipeline}
\end{example}

% However, this planning is nontrivial as there are many
% incremental computation methods to choose, but which method
% is optimal depends on the data and many other factors.
% One needs to search through the plan space of jointly different incremental methods, and the decisions
% of whether to progressively compute each subpart of a query.
The above query can be incrementally computed in many different ways.
Many factors can affect the optimal incremental plan.
Consider two basic incremental methods used in IVM and stream computing.
% Both methods can be adapted to be used to progressively compute the analytics pipeline.
%\kai{[`Batch' here emphasize we only use the algorithm not the way of execution.]}
(1)
A typical view maintenance approach \ivm{}
treats \textit{summary} as views.
% After each ingested data batch,
It always maintains \textit{summary} as if it is directly computed
from the data of \textit{sales} and \textit{returns} seen so far.
Therefore, even if a \textit{sales} order will be returned
in the future, its revenue is counted into the gross revenue temporarily.
(2)
On the contrary, a typical stream computing method \scm{}
avoids such retraction. Instead,
it holds back \textit{sales} orders that are not joined
with any \textit{returns} orders until all data is available.
Clearly, if returned orders are rare, \ivm{} can maximize
the amount of early computation and thus deliver better resource-usage plans.
Otherwise if returned orders are often, \scm{} will
avoid unnecessary recomputation caused by retraction and thus be better.
% Even for a single query, different incremental computation methods,
% including those very sophisticated ones such higher-order view maintenance~\cite{dbtoaster},
% can be jointly applied to achieve an optimal plan.
Besides incremental methods,
one further needs to trade off different physical plans
for each run in the incremental processing and consider
their correlations.
For instance, the left outer join may be implemented using
a broadcast join when \textit{returns} is very small,
but switch to a shuffled join when \textit{returns} gets larger.
However, this switching may require extra shuffles of the join
states saved in previous runs.

% First, although sharing the same processing model,
% different incremental processing applications have very diverse
% requirements and constraints.
% E.g., in IVM, the query engine must deliver the latest query result
% immediately after new data arrives, whereas in the progressive data warehouse scenario, the engine does not need to deliver any query results until the specified deadline;
% in interactive scenarios like data cleaning, the query engine
% tends to keep all necessary states in favor of query latency,
% while otherwise like in deferred IVM, the engine can tolerate
% larger update latency and can afford re-compute certain states
% when needed.

% The new progressive execution paradigm unifies different execution modes
% spanning from batch, mini-batch, to streaming execution.
% Traditional execution modes usually have a fixed execution pattern.
% For instance, view maintenance techniques always deliver the up-to-date query results
% on data seen so far; stream computing techniques always computes the delta
% on every incoming data; mini-batch techniques always computes every pre-set period.
% Progressive execution paradigm opens up a full spectrum of execution modes,
% while traditional batch and streaming execution modes are just two extreme
% example cases.

\eat{Furthermore, progressive processing introduces complex dependencies
both along the time dimension and between upstream/downstream queries in a pipeline.
For instance, in a progressive plan, previous runs
may save intermediate states to be shared by later runs.
What and how intermediate states are saved can significantly impact
the cost.
Second, modern data warehouses
typically consist of wide and deep analysis pipelines.
How a downstream query can use an early output
can affect how the upstream queries produce early outputs.
We will illustrate the details in \S\ref{sec:opt-def}.}
% First, in a plan across the time line, the subplans at each time are correlated.
% As an example, Fig.~\ref{fig:compatible-join} shows two consecutive joins when incrementally computing
% \textit{sales\_status}. Join \textcircled{2} at time $t_2$ needs to
% join both data available at $t_2$ and $t_1$.
% Thus the two joins are correlated and cannot be planned independently.
% For instance, if a previous broadcast join uses broadcast join
% while a following join use shuffled hash join,
% these two joins are not directly compatible with each other
% as the following one needs to reshuffling the data.
% Second, data analysis in modern data warehouses has complex dependencies,
% typically consisting of wide and deep pipelines.
% As we have observed at \company, the dependency chain of data analysis pipelines
% has an average depth of $xx$ jobs;
% a single analysis job is consumed by $xx$ downstream jobs on average.
% Such complexity clearly shows that any solution that only considers optimizing inside
% a single query will probably not work,
% as carrying out incremental computation for a query depends on
% its upstream queries producing proper incremental outputs.
% For instance, if the \textit{summary} query computes \texttt{MAX} aggregate
% instead of \texttt{SUM}, then the view maintenance method is not applicable
% to the \textit{sales\_status} query, as any retraction from \textit{sales\_status}
% would cause a complete recomputation of \textit{summary}.

\begin{comment}
\begin{itemize}[nosep,leftmargin=*]
  \item
  Some queries are more amendable to incremental computation while others are not.
  Even for queries that cannot be easily incrementalized, there still exists subqueries with them that can be incrementally computed.
  Therefore, one has to choose the optimal incremental computation mode for a query:
  whether we should incrementally compute the entire query or just a subpart of it,
  or simply fall back to batch execution without incremental computation.

  \item
  There are a rich body of literature on incremental computation techniques,
  ranging from various IVM techniques, to continuous or mini-batched stream computing~\cite{set-ivm-1,set-ivm-2,outerjoin-view,batch-dbtoaster,dbtoaster,dstream}.
  Each technique has its best application queries.
  Therefore, one has to pick the optimal incremental computation technique for
  a query, or even for each subpart of the query.
  % Traditional incremental computation usually has a fixed, relatively simple
  % execution pattern, e.g., stream computing is required to constantly deliver
  % results on the data seen so far; view maintenance has to always make sure
  % the content view up to date as if it is computed on the data seen so far.
  % On the contrary, progressive execution does not have a fixed execution pattern,
  % the early execution can choose deliver results in any form, or even choose to not
  % deliver any results. Therefore, progressive execution can choose in a much larger
  % plan space.

  \item
  Data ingestion is not uniform across the time line. At different time,
  the data ingestion rate may be different, and the distribution of the ingested data may be different.
  Therefore, one has to plan according to the size and distribution of data,
  which may result in different optimal query plan.
  Furthermore, the planning across the time line is correlated,
  as each execution may rely on its previous execution to save certain states that is necessary for incremental computation.
  % Similar to traditional incremental computation, progressive execution has to consider
  % across the time line and plan for the future. However, as the execution time is not
  % fixed, and the incremental plans can change at different execution instances,
  % progressive execution has to deal with much higher complexity.

  \item
  % Progressive execution has to also consider complex dependencies across
  % multiple queries, as downstream queries rely on the early execution output
  % of upstream queries. Progressive execution is no longer a single-query optimization
  % problem, but a multi-query one.
  Last but not least, data analysis in modern data warehouses has complex dependencies,
  typically consisting of wide and deep pipelines.
  % e.g., pipelines of ETL-like jobs like intensive data integration, cleaning and so on,
  % followed by pipelines of analysis on various aspects.
  As we have observed in \company{}, the dependency chain of data analysis pipelines
  has an average depth of $xx$ jobs;
  a single analysis job is consumed by $xx$ downstream jobs on average.
  Such complexity clearly shows that any solution that only considers optimizing inside
  a single query will probably not work,
  as carrying out incremental computation for a query depends on
  its upstream queries producing proper incremental outputs.
\end{itemize}
\end{comment}

\eat{The above discussion clearly demonstrates the complexity of planning progressive processing.
It needs to jointly plan along three dimensions:
% (1) different incremental modes,
(1) different incremental computation techniques,
(2) data characteristics such distribution and arrival rate,
% (3) different execution instances along the time dimension, and
and (3) complex dependencies along the time line and across queries.
Such planning has to be done in a cost-based manner.
However, existing theory and systems for query optimization
are usually only able to explore the plan space of a query at a single time point,
using a single fixed execution mode or computation method, either normal execution or a fixed incremental computation method.
A progressive processing paradigm needs new theories and systems for query planning.}

% \begin{figure}[htb!]
% \centering
% \tiny
% \begin{tabular}{cc}
% \subfigure[]{
% 	\begin{tabular}{|c|c|c|c|c}
% 	\cline{1-4}
% 	\texttt{order\_no} & \texttt{store\_no} & \texttt{total} & \texttt{promo\_no} & \\
% 	\cline{1-4}
% 	$o_1$ & $s_1$ & $100$ & $p_1$ & $t_1$ \\
% 	\cline{1-4}
% 	$o_2$ & $s_2$ & $200$ & $p_2$ & $t_1$ \\
% 	\cline{1-4}
% 	$o_3$ & $s_1$ & $300$ & $p_2$ & $t_2$ \\
% 	\cline{1-4}
% 	\end{tabular}
%   \label{fig:ex-sales}
% }
% &
% \subfigure[]{
%   \begin{tabular}{|c|c|c}
%   \cline{1-2}
%   \texttt{promo\_no} & \texttt{discount} & \\
%   \cline{1-2}
%   $p_1$ & $0.9$ & $t_1$ \\
%   \cline{1-2}
%   $p_2$ & $0.8$ & $t_2$ \\
%   \cline{1-2}
%   \end{tabular}
%   \label{fig:ex-promo}
% }
% \\
% \subfigure[]{
%   \begin{tabular}{|c|c|c|c|}
%   \hline
%   \texttt{order\_no} & \texttt{store\_no} & \texttt{total} & \texttt{discount} \\
%   \hline
%   $o_1$ & $s_1$ & $100$ & $0.9$ \\
%   \hline
%   $o_2$ & $s_2$ & $200$ & $null$ \\
%   \hline
%   \end{tabular}
%   \label{fig:ext_sales-retract}
% }
% &
% \subfigure[]{
%   \begin{tabular}{|c|c|}
%   \hline
%   \texttt{store\_no} & \texttt{SUM} \\
%   \hline
%   $s_1$ & $90$ \\
%   \hline
%   $s_2$ & $200$ \\
%   \hline
%   \end{tabular}
%   \label{fig:summary-retract}
% }
% \\
% \subfigure[]{
%   \begin{tabular}{|c|c|c|c|}
%   \hline
%   \texttt{order\_no} & \texttt{store\_no} & \texttt{total} & \texttt{discount} \\
%   \hline
%   $o_1$ & $s_1$ & $100$ & $0.9$ \\
%   \hline
%   \end{tabular}
%   \label{fig:ex-no-retract}
% }
% &
% \subfigure[]{
%  \begin{tabular}{|c|c|}
%   \hline
%   \texttt{store\_no} & \texttt{SUM} \\
%   \hline
%   $s_1$ & $90$ \\
%   \hline
%   \end{tabular}
%   \label{fig:summary-no-retract}
% }
% \\
% \subfigure[]{
%   \begin{tabular}{|c|c|c|c|}
%   \hline
%   \texttt{order\_no} & \texttt{store\_no} & \texttt{total} & \texttt{discount} \\
%   \hline
%   $o_1$ & $s_1$ & $100$ & $0.9$ \\
%   \hline
%   $o_2$ & $s_2$ & $200$ & $0.8$ \\
%   \hline
%   $o_3$ & $s_1$ & $300$ & $0.8$ \\
%   \hline
%   \end{tabular}
%   \label{fig:ext_sales-full}
% }
% &
% \subfigure[]{
%   \begin{tabular}{|c|c|}
%   \hline
%   \texttt{store\_no} & \texttt{SUM} \\
%   \hline
%   $s_1$ & $330$ \\
%   \hline
%   $s_2$ & $160$ \\
%   \hline
%   \end{tabular}
%   \label{fig:summary-full}
% }
% \end{tabular}
% \caption{(a)(b) Data arrival of \texttt{sales} and \texttt{promotions} respectively;
% (c)(d) early results of \texttt{ext\_sales} and \texttt{summary} at $t_1$ produced by
% the view maintenance method;
% (e)(f) early results of \texttt{ext\_sales} and \texttt{summary} at $t_1$ produced by
% the stream computing method;
% (g)(h) full results of \texttt{ext\_sales} and \texttt{summary} at $t_2$}
% \label{fig:all-tvr-ex}
% \end{figure}

% \noindent
% \textbf{Query Optimization}.
% The new progressive execution paradigm utilizes incremental computation.
% Although extensively studied in various areas
% such as including view maintenance, stream computing,
% and so on~\cite{bag-ivm-1,bag-ivm-2,dbtoaster,cql},
% previously incremental computation is mostly studied in isolation.
% In different areas, incremental computation takes different forms;
% and in practice, there is no principled solution to find out
% for a specific scenario whether to use incremental computation and
% which incremental computation technique delivers optimal performance.
% A manual solution is very challenging even for experienced engineers
% and error prone.
% Actually among different incremental computation approaches,
% no one can always deliver better performance than others;
% the optimal incremental computation plan, or even whether to use incremental computation
% or not, is query dependent and data dependent.
% Different techniques should be unified and applied together in query plans,
% and the optimal plan can be searched by system automatically in a cost-based way.
% The following example demonstrate exactly this point.
% Fig.~\ref{fig:ex-sales} and~\ref{fig:ex-promo} show
% an append-only example of \texttt{sales} and \texttt{promotions}.
% Suppose both tables are fully collected at $t_2$, but the system would like to
% execute Example~\ref{ex:running} early at $t_2$ with partial data.
% As appends to \texttt{sales} and \texttt{promotions} are not synchronized,
% it is possible that we see an order (e.g., $(o_2, s_1, 200, p_2)$ at $t_1$)
% before we see its corresponding promotion campaign (e.g., $(p_2, 0.8)$ at $t_2$).
% To execute \texttt{ext\_sales} early at $t_1$:
% the view maintenance approach simply computes the outer join in \texttt{ext\_sales}
% as is on \texttt{sales} and \texttt{promotions} at $t_1$, which generates
% as many early outputs as possible, but may have to retract some of the outputs later,
% e.g., tuple $o_2$ in Fig.~\ref{fig:ext_sales-retract}, as they are not part of the final results
% as shown in Fig.~\ref{fig:ext_sales-full};
% on the contrary, the stream computing way only outputs join tuples that are surely
% part of the final results---essentially the inner join of \texttt{sales} and \texttt{promotions} at $t_1$---as shown in Fig.~\ref{fig:ex-no-retract}.
% Which approach delivers better performance is data dependent:
% if the updates to both tables are mostly synchronized and retraction is rare,
% the view maintenance is better as it can generates more early results
% and let \texttt{summary} carry out more early computation;
% if most early outputs may be retracted, the stream computing way
% is better as retraction will waste computation anyway.
% What is more, this decision also depends on interaction with other queries:
% Consider a different \texttt{summary} with \texttt{MAX} instead of \texttt{SUM}.
% Retraction in \texttt{ext\_sales} is not allowed as each tuple retracted can
% cause \texttt{MAX} to recompute from scratch.

The above example clearly shows that
incremental query planning is more challenging than
the traditional query planning:
(1)
\emph{Besides the traditional dimensions including algebra-equivalent
rewritings, implementations of relational operators,
ways of data retrieval methods, and data statistics,
incremental query planning needs to further trade off
between different incremental computation methods,
data arrival patterns, which states to materialize.}
(2) \emph{The plans for each incremental run are correlated.}
In this paper,
we propose a unified cost-based query optimization framework, which allows users to express and integrate various incremental computation techniques
and provides a turn-key solution to decide optimal progressive execution plans
subject to various objectives.
We propose a theory called \emph{time-varying relation model}
for modeling incremental processing.
It naturally extends the relational model by considering the temporal aspect,
modeling changing data as a time-varying relation (TVR),
with snapshots and deltas as two different views of encoding a TVR.
It also includes various data-manipulation operations on TVR's,
as well as TVR rewriting rules.
It provides a general framework for a query optimizer
to define various incremental computation techniques,
and unifies them to explore a search space to generate an efficient execution plan.
This model allows various incremental computation techniques to work cooperatively,
and enables cost-based search among all possible incremental plans.

We demonstrate how to support
cost-based progressive planning
by incorporating the TVR model on a Cascade-style
optimizer, and build a prototype optimizer named~\sys{}.\footnote{The name of the system is based on the shape of the query-plan representation.  It is also consistent with the ``magic'' nature of this general optimizer framework.}
Our key contributions are:
% We implemented this framework based on calcite---a volcano optimizer,
% and used it inside our \company{} enterprise-scale data warehouse.
% Therefore, our focus is on the volcano framework that enables the search,
% not delta computation itself.
\begin{itemize}[nosep,leftmargin=*]
  \item We propose a new theory called time-varying relation model that can formally model progressive execution in its most general form (\S\ref{sec:model}),
  and provide a general framework for a query optimizer to define and unify various incremental computation techniques
  to jointly explore a search space for an efficient progressive plan (\S\ref{sec:tvr-rules}).

  \item We build a Cascade-style optimizer named \sys{} that incorporates the TVR model, and supports cost-based optimization for progressive planning.
  % \sys{} incorporates the TVR model and support exploration and search in a plan space spanning
  % four dimensions, including different incremental modes, different incremental computation methods, across the time line and different queries.
  We discuss how to explore the plan space (\S\ref{sec:plan-space-exploration}) and select an optimal  progressive plan (\S\ref{sec:select-a-plan}) in \sys{}.
  %   We introduce speed-up optimizations to enable
  % efficient exploration of a much bigger plan space
  % along different incremental modes, different incremental computation methods,
  % across the time line and different queries.
  % We also develop novel costing and searching algorithms
  % to search through the plan space for the optimal plan
  % with the ability to fully exploit sharing opportunities across time
  % and a entire analysis pipeline consisting of multiple queries.

  \item We study experimentally the \sys{} optimizer
  in various application scenarios.
  The experimental results show the effectiveness and efficiency
  of \sys{} in planning incremental execution (\S\ref{sec:experiments}).
\end{itemize}

% The rest of this paper is organized as follows. We discuss related work in Section~\ref{sec:related} and conclude in Section~\ref{sec:conclusion}.


==> leftover.tex <==

\section{Leftover materials from Section 1: Introduction}



% First, although sharing the same processing model,
% different incremental processing applications have very diverse
% requirements and constraints.
% E.g., in IVM, the query engine must deliver the latest query result
% immediately after new data arrives, whereas in the progressive data warehouse scenario, the engine does not need to deliver any query results until the specified deadline;
% in interactive scenarios like data cleaning, the query engine
% tends to keep all necessary states in favor of query latency,
% while otherwise like in deferred IVM, the engine can tolerate
% larger update latency and can afford re-compute certain states
% when needed.

% The new progressive execution paradigm unifies different execution modes
% spanning from batch, mini-batch, to streaming execution.
% Traditional execution modes usually have a fixed execution pattern.
% For instance, view maintenance techniques always deliver the up-to-date query results
% on data seen so far; stream computing techniques always computes the delta
% on every incoming data; mini-batch techniques always computes every pre-set period.
% Progressive execution paradigm opens up a full spectrum of execution modes,
% while traditional batch and streaming execution modes are just two extreme
% example cases.

\eat{Furthermore, progressive processing introduces complex dependencies
both along the time dimension and between upstream/downstream queries in a pipeline.
For instance, in a progressive plan, previous runs
may save intermediate states to be shared by later runs.
What and how intermediate states are saved can significantly impact
the cost.
Second, modern data warehouses
typically consist of wide and deep analysis pipelines.
How a downstream query can use an early output
can affect how the upstream queries produce early outputs.
We will illustrate the details in \S\ref{sec:opt-def}.}
% First, in a plan across the time line, the subplans at each time are correlated.
% As an example, Fig.~\ref{fig:compatible-join} shows two consecutive joins when incrementally computing
% \textit{sales\_status}. Join \textcircled{2} at time $t_2$ needs to
% join both data available at $t_2$ and $t_1$.
% Thus the two joins are correlated and cannot be planned independently.
% For instance, if a previous broadcast join uses broadcast join
% while a following join use shuffled hash join,
% these two joins are not directly compatible with each other
% as the following one needs to reshuffling the data.
% Second, data analysis in modern data warehouses has complex dependencies,
% typically consisting of wide and deep pipelines.
% As we have observed at \company, the dependency chain of data analysis pipelines
% has an average depth of $xx$ jobs;
% a single analysis job is consumed by $xx$ downstream jobs on average.
% Such complexity clearly shows that any solution that only considers optimizing inside
% a single query will probably not work,
% as carrying out incremental computation for a query depends on
% its upstream queries producing proper incremental outputs.
% For instance, if the \textit{summary} query computes \texttt{MAX} aggregate
% instead of \texttt{SUM}, then the view maintenance method is not applicable
% to the \textit{sales\_status} query, as any retraction from \textit{sales\_status}
% would cause a complete recomputation of \textit{summary}.

\begin{comment}
\begin{itemize}[nosep,leftmargin=*]
  \item
  Some queries are more amendable to incremental computation while others are not.
  Even for queries that cannot be easily incrementalized, there still exists subqueries with them that can be incrementally computed.
  Therefore, one has to choose the optimal incremental computation mode for a query:
  whether we should incrementally compute the entire query or just a subpart of it,
  or simply fall back to batch execution without incremental computation.

  \item
  There are a rich body of literature on incremental computation techniques,
  ranging from various IVM techniques, to continuous or mini-batched stream computing~\cite{set-ivm-1,set-ivm-2,outerjoin-view,batch-dbtoaster,dbtoaster,dstream}.
  Each technique has its best application queries.
  Therefore, one has to pick the optimal incremental computation technique for
  a query, or even for each subpart of the query.
  % Traditional incremental computation usually has a fixed, relatively simple
  % execution pattern, e.g., stream computing is required to constantly deliver
  % results on the data seen so far; view maintenance has to always make sure
  % the content view up to date as if it is computed on the data seen so far.
  % On the contrary, progressive execution does not have a fixed execution pattern,
  % the early execution can choose deliver results in any form, or even choose to not
  % deliver any results. Therefore, progressive execution can choose in a much larger
  % plan space.

  \item
  Data ingestion is not uniform across the time line. At different time,
  the data ingestion rate may be different, and the distribution of the ingested data may be different.
  Therefore, one has to plan according to the size and distribution of data,
  which may result in different optimal query plan.
  Furthermore, the planning across the time line is correlated,
  as each execution may rely on its previous execution to save certain states that is necessary for incremental computation.
  % Similar to traditional incremental computation, progressive execution has to consider
  % across the time line and plan for the future. However, as the execution time is not
  % fixed, and the incremental plans can change at different execution instances,
  % progressive execution has to deal with much higher complexity.

  \item
  % Progressive execution has to also consider complex dependencies across
  % multiple queries, as downstream queries rely on the early execution output
  % of upstream queries. Progressive execution is no longer a single-query optimization
  % problem, but a multi-query one.
  Last but not least, data analysis in modern data warehouses has complex dependencies,
  typically consisting of wide and deep pipelines.
  % e.g., pipelines of ETL-like jobs like intensive data integration, cleaning and so on,
  % followed by pipelines of analysis on various aspects.
  As we have observed in \company{}, the dependency chain of data analysis pipelines
  has an average depth of $xx$ jobs;
  a single analysis job is consumed by $xx$ downstream jobs on average.
  Such complexity clearly shows that any solution that only considers optimizing inside
  a single query will probably not work,
  as carrying out incremental computation for a query depends on
  its upstream queries producing proper incremental outputs.
\end{itemize}
\end{comment}

\eat{The above discussion clearly demonstrates the complexity of planning progressive processing.
It needs to jointly plan along three dimensions:
% (1) different incremental modes,
(1) different incremental computation techniques,
(2) data characteristics such distribution and arrival rate,
% (3) different execution instances along the time dimension, and
and (3) complex dependencies along the time line and across queries.
Such planning has to be done in a cost-based manner.
However, existing theory and systems for query optimization
are usually only able to explore the plan space of a query at a single time point,
using a single fixed execution mode or computation method, either normal execution or a fixed incremental computation method.
A progressive processing paradigm needs new theories and systems for query planning.}

% \begin{figure}[htb!]
% \centering
% \tiny
% \begin{tabular}{cc}
% \subfigure[]{
% 	\begin{tabular}{|c|c|c|c|c}
% 	\cline{1-4}
% 	\texttt{order\_no} & \texttt{store\_no} & \texttt{total} & \texttt{promo\_no} & \\
% 	\cline{1-4}
% 	$o_1$ & $s_1$ & $100$ & $p_1$ & $t_1$ \\
% 	\cline{1-4}
% 	$o_2$ & $s_2$ & $200$ & $p_2$ & $t_1$ \\
% 	\cline{1-4}
% 	$o_3$ & $s_1$ & $300$ & $p_2$ & $t_2$ \\
% 	\cline{1-4}
% 	\end{tabular}
%   \label{fig:ex-sales}
% }
% &
% \subfigure[]{
%   \begin{tabular}{|c|c|c}
%   \cline{1-2}
%   \texttt{promo\_no} & \texttt{discount} & \\
%   \cline{1-2}
%   $p_1$ & $0.9$ & $t_1$ \\
%   \cline{1-2}
%   $p_2$ & $0.8$ & $t_2$ \\
%   \cline{1-2}
%   \end{tabular}
%   \label{fig:ex-promo}
% }
% \\
% \subfigure[]{
%   \begin{tabular}{|c|c|c|c|}
%   \hline
%   \texttt{order\_no} & \texttt{store\_no} & \texttt{total} & \texttt{discount} \\
%   \hline
%   $o_1$ & $s_1$ & $100$ & $0.9$ \\
%   \hline
%   $o_2$ & $s_2$ & $200$ & $null$ \\
%   \hline
%   \end{tabular}
%   \label{fig:ext_sales-retract}
% }
% &
% \subfigure[]{
%   \begin{tabular}{|c|c|}
%   \hline
%   \texttt{store\_no} & \texttt{SUM} \\
%   \hline
%   $s_1$ & $90$ \\
%   \hline
%   $s_2$ & $200$ \\
%   \hline
%   \end{tabular}
%   \label{fig:summary-retract}
% }
% \\
% \subfigure[]{
%   \begin{tabular}{|c|c|c|c|}
%   \hline
%   \texttt{order\_no} & \texttt{store\_no} & \texttt{total} & \texttt{discount} \\
%   \hline
%   $o_1$ & $s_1$ & $100$ & $0.9$ \\
%   \hline
%   \end{tabular}
%   \label{fig:ex-no-retract}
% }
% &
% \subfigure[]{
%  \begin{tabular}{|c|c|}
%   \hline
%   \texttt{store\_no} & \texttt{SUM} \\
%   \hline
%   $s_1$ & $90$ \\
%   \hline
%   \end{tabular}
%   \label{fig:summary-no-retract}
% }
% \\
% \subfigure[]{
%   \begin{tabular}{|c|c|c|c|}
%   \hline
%   \texttt{order\_no} & \texttt{store\_no} & \texttt{total} & \texttt{discount} \\
%   \hline
%   $o_1$ & $s_1$ & $100$ & $0.9$ \\
%   \hline
%   $o_2$ & $s_2$ & $200$ & $0.8$ \\
%   \hline
%   $o_3$ & $s_1$ & $300$ & $0.8$ \\
%   \hline
%   \end{tabular}
%   \label{fig:ext_sales-full}
% }
% &
% \subfigure[]{
%   \begin{tabular}{|c|c|}
%   \hline
%   \texttt{store\_no} & \texttt{SUM} \\
%   \hline
%   $s_1$ & $330$ \\
%   \hline
%   $s_2$ & $160$ \\
%   \hline
%   \end{tabular}
%   \label{fig:summary-full}
% }
% \end{tabular}
% \caption{(a)(b) Data arrival of \texttt{sales} and \texttt{promotions} respectively;
% (c)(d) early results of \texttt{ext\_sales} and \texttt{summary} at $t_1$ produced by
% the view maintenance method;
% (e)(f) early results of \texttt{ext\_sales} and \texttt{summary} at $t_1$ produced by
% the stream computing method;
% (g)(h) full results of \texttt{ext\_sales} and \texttt{summary} at $t_2$}
% \label{fig:all-tvr-ex}
% \end{figure}

% \noindent
% \textbf{Query Optimization}.
% The new progressive execution paradigm utilizes incremental computation.
% Although extensively studied in various areas
% such as including view maintenance, stream computing,
% and so on~\cite{bag-ivm-1,bag-ivm-2,dbtoaster,cql},
% previously incremental computation is mostly studied in isolation.
% In different areas, incremental computation takes different forms;
% and in practice, there is no principled solution to find out
% for a specific scenario whether to use incremental computation and
% which incremental computation technique delivers optimal performance.
% A manual solution is very challenging even for experienced engineers
% and error prone.
% Actually among different incremental computation approaches,
% no one can always deliver better performance than others;
% the optimal incremental computation plan, or even whether to use incremental computation
% or not, is query dependent and data dependent.
% Different techniques should be unified and applied together in query plans,
% and the optimal plan can be searched by system automatically in a cost-based way.
% The following example demonstrate exactly this point.
% Fig.~\ref{fig:ex-sales} and~\ref{fig:ex-promo} show
% an append-only example of \texttt{sales} and \texttt{promotions}.
% Suppose both tables are fully collected at $t_2$, but the system would like to
% execute Example~\ref{ex:running} early at $t_2$ with partial data.
% As appends to \texttt{sales} and \texttt{promotions} are not synchronized,
% it is possible that we see an order (e.g., $(o_2, s_1, 200, p_2)$ at $t_1$)
% before we see its corresponding promotion campaign (e.g., $(p_2, 0.8)$ at $t_2$).
% To execute \texttt{ext\_sales} early at $t_1$:
% the view maintenance approach simply computes the outer join in \texttt{ext\_sales}
% as is on \texttt{sales} and \texttt{promotions} at $t_1$, which generates
% as many early outputs as possible, but may have to retract some of the outputs later,
% e.g., tuple $o_2$ in Fig.~\ref{fig:ext_sales-retract}, as they are not part of the final results
% as shown in Fig.~\ref{fig:ext_sales-full};
% on the contrary, the stream computing way only outputs join tuples that are surely
% part of the final results---essentially the inner join of \texttt{sales} and \texttt{promotions} at $t_1$---as shown in Fig.~\ref{fig:ex-no-retract}.
% Which approach delivers better performance is data dependent:
% if the updates to both tables are mostly synchronized and retraction is rare,
% the view maintenance is better as it can generates more early results
% and let \texttt{summary} carry out more early computation;
% if most early outputs may be retracted, the stream computing way
% is better as retraction will waste computation anyway.
% What is more, this decision also depends on interaction with other queries:
% Consider a different \texttt{summary} with \texttt{MAX} instead of \texttt{SUM}.
% Retraction in \texttt{ext\_sales} is not allowed as each tuple retracted can
% cause \texttt{MAX} to recompute from scratch.







% The solution we propose is a full-fledged data warehouse solution
% based on a new execution paradigm---\emph{progressive execution}.
% The key idea is that, instead of letting all queries wait until
% their registered scheduling time, when all their input data are ready,
% whenever the data warehouse finds that the cluster has free resources,
% it can choose queries part of whose input data are ready to execute earlier,
% in order to utilize the resource.
% The early execution consumes the existing input data and saves necessary state
% for future processing of the up-coming input data, which essentially moves
% part of the computation work required off the traffic hour of the cluster,
% to a less congested time, and reduces the delivery latency of the query answer;
% it also optionally generates early outputs (not necessarily the query results),
% which in turns unblocks the downstream queries depending on it,
% so that the data warehouse can choose to early execute them later.
% Furthermore, the data warehouse can always kill an early execution
% when it sees urgent resource requirement, as the early execution is anyway speculative.
% In short, the progressive execution enable engines to execute a query at any time
% on any subset of the input data,
% and to pause and pick up the dropped-off work as wanted at any time.
% Clearly, this execution paradigm dovetails the merits of both batch and
% streaming processing paradigms:
% (1) similar to streaming computing, it enables more timely processing of accumulated
% input data and reduces the query latency,
% (2) it still processes data in a batch way during early execution with high throughput,
% but without holding resources unnecessarily,
% (3) it allows much flexible scheduling, and enables peak loads shifting,
% significantly optimizes the resource utilization of the cluster.
% \kai{[From users' perspective, better resource utilization means less resource provision
% for their analysis jobs, which leads to lower risks for missing deadlines,
% and lower resource bills.]}

% To depict the progressive execution paradigm, consider the following example
% OLAP pipeline consists of a data integration job (\texttt{ext\_sales})
% followed by an aggregation analysis (\texttt{summary}).
% \begin{example}
% \begin{alltt}
%     \small
%    ext_sales =
%     SELECT order_no, store_no, total, discount
%     FROM sales LEFT OUTER JOIN promotions
%          ON sales.promo_no=promotions.promo_no

%    summary =
%     SELECT store_no,
%       SUM(IF(discount is NULL, total, total*discount))
%     FROM ext_sales
%     GROUP BY store_no
% \end{alltt}
% \label{ex:running}
% \end{example}
% \begin{figure}[htb!]
% \centering
% \includegraphics[width=0.45\textwidth]{figs/timeline.png}
% \caption{How Example~\ref{ex:running} executes in traditional data warehouses vs \sys}
% \label{fig:timeline}
% \end{figure}
% Fig.~\ref{fig:timeline} compares how Example~\ref{ex:running} are executed
% in a traditional data warehouse and in our data warehouse \sys~on a timeline.
% Traditionally, even the data of \texttt{sales}
% and \texttt{promotions} are constantly ingested into the data warehouse
% and most is available way before the scheduled job time (at $12$am of day$2$),
% the system cannot execute \texttt{ext\_sales} and \texttt{summary},
% even though the cluster has available capacities.
% Differently \sys~can start executing \texttt{ext\_sales}
% when part of \texttt{sales} and \texttt{promotions} are available,
% and the cluster has available capacities (at $6$am, $12$pm and $18$pm of day$1$).
% Each execution can resume from the work left by the previous execution,
% and the final execution at $12$am of day$2$ finishes much faster.
% Furthermore, the early outputs of \texttt{ext\_sales} in turn
% enables the \texttt{aggregation} query to execute early too.
% Although progressive execution seems similar to traditional
% incremental computation such as view maintenance and stream computing,
% key questions in progressive execution, such as
% finding the cost-optimal progressive query plans and deciding
% when to run what queries, have significant complexity and challenges
% that are not tackled in previous research.
% This opens up a whole new line of research, and
% requires us to rethink the techniques of data warehouses,
% from query optimization to job scheduling and resource management.

% \begin{figure}[htb!]
% \centering
% \includegraphics[width=0.5\textwidth]{figs/paradigm-comparison.jpg}
% \caption{Comparison of progressive computation, stream computation and batch computation}
% \label{fig:pattern-comparison}
% \end{figure}

\eat{
Astute readers may think, ``isn't this just another form of incremental computation?''
The answer is ``yes''. Indeed, there is a rich body of research work
on various forms of incremental computation, ranging from incremental view maintenance (IVM), stream computing, to approximate/interactive query answering and so on.
However, previously these incremental techniques are
mostly studied in isolation. But as we will show below, it is a nontrivial problem
to figure out the optimal progressive execution plan exploiting these techniques.
Rather than proposing yet another incremental computation technique,
we are focusing on a unified cost-based query optimization framework
that can allow users to express and integrate various incremental computation techniques
and provide turn-key solution to decide the optimal progressive execution plans
subject to various objectives.
}

% Astute readers may think, ``isn't this just another form of incremental view maintenance (IVM)?''
% % A straightforward solution would be to adopt a small-batched solution:
% That is, one can treat a routine analysis query as a view to maintain.
% The ingested data is just updates to base relations
% % accumulated up to certain batch size or time interval,
% and triggers refresh on the view using incremental computation.
% % In this way, we do not need to wait until the scheduled time to compute
% % the analysis, but scatter the computation across the day,
% % alleviating the resource pressure on the traffic hour.
% However, this is only partially right.
% The core of progressive processing does rely on incremental computation techniques,
% but planning progressive processing is not as trivial as it looks like.
% % Progressive execution paradigm greatly extends the traditional
% % batch and streaming computation paradigms.
% % The key difference is that progressive execution can flexibly
% % schedule early execution of queries on any partial input data at any time.
% % Fig.~\ref{fig:pattern-comparison} depicts the execution patterns of the three execution paradigms.


% We propose a theory called \emph{time-varying relation model}
% for modeling incremental processing in its most general form.
% It naturally extends the relational model by considering the temporal aspect,
% modeling changing data as a time-varying relation (TVR),
% with snapshots and deltas as two different views of encoding a TVR.
% It also includes various data-manipulation operations on TVR's,
% as well as TVR rewriting rules.
% It provides a general framework for a query optimizer
% to define various incremental computation techniques,
% and unifies them to explore a search space to generate an efficient execution plan.





% We demonstrate how to support
% cost-based progressive planning
% by incorporating the TVR model on a Cascade-style
% optimizer, and build a prototype optimizer named \sys{}.

% We implemented this framework based on calcite---a volcano optimizer,
% and used it inside our \company{} enterprise-scale data warehouse.
% Therefore, our focus is on the volcano framework that enables the search,
% not delta computation itself.
% \begin{itemize}[nosep,leftmargin=*]
%   \item We propose a new theory called time-varying relation model that can formally model progressive execution in its most general form (\S\ref{sec:model}),
%   and provide a general framework for a query optimizer to define and unify various incremental computation techniques
%   to jointly explore a search space for an efficient progressive plan (\S\ref{sec:tvr-rules}).

%   \item We build a Cascade-style optimizer named \sys{} that incorporates the TVR model, and supports cost-based optimization for progressive planning.
%   % \sys{} incorporates the TVR model and support exploration and search in a plan space spanning
%   % four dimensions, including different incremental modes, different incremental computation methods, across the time line and different queries.
%   We discuss how to explore the plan space (\S\ref{sec:plan-space-exploration}) and select an optimal  progressive plan (\S\ref{sec:select-a-plan}) in \sys{}.
%   %   We introduce speed-up optimizations to enable
%   % efficient exploration of a much bigger plan space
%   % along different incremental modes, different incremental computation methods,
%   % across the time line and different queries.
%   % We also develop novel costing and searching algorithms
%   % to search through the plan space for the optimal plan
%   % with the ability to fully exploit sharing opportunities across time
%   % and a entire analysis pipeline consisting of multiple queries.

%   \item We study experimentally the \sys{} optimizer
%   in various application scenarios.
%   The experimental results show the effectiveness and efficiency
%   of \sys{} in planning incremental execution (\S\ref{sec:experiments}).
% \end{itemize}

% The rest of this paper is organized as follows. We discuss related work in Section~\ref{sec:related} and conclude in Section~\ref{sec:conclusion}.


\section{From Section 2}

% Consider a warehouse with data arriving continuously, and a set of queries that need to be executed at certain times.   Each query is expected to run at a specific time $T$
% on the data collected in a time window that ends at $T$.  The data warehouse has a computing cluster whose resource usage fluctuates over time, i.e., sometimes it is heavily used and sometimes there are many idle resources.  The warehouse monitors its cluster usage and the data-ingestion rate.  Whenever it finds that the cluster has free resources, or some queries have enough arrived data, it selects one or more queries (referred to as a workflow $W$)
% from the registered queries, and proposes a {\em schedule} $S$ to run this workflow.
% The schedule includes a set of time points on which we want to run $W$ progressively.
% Our goal is to do a cost-based analysis and generate a progressive plan to run the query incrementally at those times.  Formally, we are given the following:
% \begin{itemize}[nosep,leftmargin=*]
%  \item A workflow $W$ consisting one or more queries.

%  \item A schedule $S=\{t_0, t_1, \ldots, t_n, t^*\}$, where $t_0$ is the current time, and $t^*$ is the final time of finishing $W$, i.e., the max of the specified execution time $T$ of each query in $W$.

%  \item The input data available at each time $t_i$, e.g., the newly available data at time $t_i$, or early output generated from upstream queries.
% % Note that the statistics of the input data usually can be obtained from the past executed queries as many queries in the data warehouse are repeated (e.g., run once every day).

%  % \item Other dependency information, such as  saved states of previous runs of the query (provided in as materialized views), and downstream dependent queries. \hl{CL: it's a bit vague.}

% \end{itemize}

% Our goal is to generate a progressive plan for the schedule.
% A progressive plan consists of a sequence of physical plan $\pl = [P_0, P_1, \cdots, P_n]$,
% where $P_i$ defines the task to execute at time $t_i$.
% Compared to a traditional physical plan, $P_i$ can include decisions of
% materializing intermediate states at $t_i$ to share for later runs.
% A proposed schedule can be tentative and subject to change.
% Once the schedule changes, we can re-plan for the new schedule
% by taking into account the partially executed progressive plan of the old schedule.
% We will discuss these advanced planning issues in \S\ref{sec:discussion}.

% \begin{definition}[Progressive Query Planning]
% Given a (or a DAG of) query(ies), $T$ time points to consider ($t_1\cdots t_T$),
% and one or several required output nodes (referred to as the \emph{target nodes}) at certain time points (e.g. $C$ at $t_3$, or $C_3$),
% the cross-time plan space is a directed graph which contains the full set of possible
% TVR transformations defined by the given rules, expanded with their possible execution time.
% Our goal is to extend the volcano framework to search for the best cross-time plan $P$ that:
% 1. produces all targets nodes at the required time points,
% and 2. minimizes an overall score function
% $\mathbb{C}(P) = \mathbb{C}(c_1(P), \cdots, c_T(P))$, where $c_i(P)$ is the estimated execution cost of the sub-plan at time $t_i$.
% \end{definition}

% Problem formulation:
% \emph{Provide a few execution time points and various forms of input
% relations available at the corresponding time points,
% as well as one or more output requirements, find the optimal plan.}

% In this work, we propose a heuristic-based end-to-end solution as a first step towards the full problem.
% Here are some basic ideas:

% \begin{enumerate}

% \item Unify multi-query and single query case: merge multiple queries into a single large query and optimize as a whole.
% Unify the exploration and optimization of sharing opportunities within and across queries.

% \item Whenever the cluster has spare capacity, it is an opportunity to progressively do some work,
% otherwise the cluster resource is left idle and wasted anyway.

% \item When planning, we only consider two time points: now (when the cluster has spare capacity)
% and the future final run when the full result is needed.
% This allows us to avoid the extra complexity and uncertainty brought by the multiple future steps.

% \item Since the current resource is considered free,
% we use the score function that strictly prefer early execution (see (c) in \S\ref{sec:opt-def}).
% As we will show later, in this case there is no need to expand the cross-time plan space by execution time.
% \end{enumerate}


%!TEX root=main.tex




% Compared to previous research which studies incremental computation in isolation
% in various settings, such as view maintenance, stream computing,
% approximate/interactive query answering and so on,
% this flexibility opens up a much larger and challenging plan space
% for progressive planning to trade-off,
% the new trade-off dimensions include:
% (1) whether the query should be progressively computed,
% (2) whether to output early results, and what kind of early results to output,
% (3) how the downstream would use the early results, and
% (4) which incremental computation method to use.


%{\bf CL: It opens up a much larger plan space for progressive planning to trade-off when jointly consider different incremental computation techniques, different data characteristics and complex dependencies along time and across queries, for which cost-based optimization becomes essential for finding the optimal progressive plan.}



\begin{comment}
\begin{figure*}[thb!]
\centering
\tiny
\begin{tabular}{cc;{2pt/2pt}cc;{2pt/2pt}cc}
\multirow{6}{*}{
  \subfigure[]{
    \includegraphics[width=0.059\textwidth]{figs/plan.pdf}
  }
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|c}
  \cline{1-3}
  \textit{o\_id} & \textit{cat} & \textit{price} & \\
  \cline{1-3}
  $o_1$ & $c_1$ & $100$ & $t_1$ \\
  \cline{1-3}
  $o_2$ & $c_2$ & $150$ & $t_1$ \\
  \cline{1-3}
  $o_3$ & $c_1$ & $120$ & $t_1$ \\
  \cline{1-3}
  $o_4$ & $c_1$ & $170$ & $t_1$ \\
  \cline{1-3}
  $o_5$ & $c_2$ & $300$ & $t_2$ \\
  \cline{1-3}
  $o_6$ & $c_1$ & $150$ & $t_2$ \\
  \cline{1-3}
  $o_7$ & $c_2$ & $220$ & $t_2$ \\
  \cline{1-3}
  \end{tabular}
  \label{fig:sales}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{price} \\
  \hline
  $o_1$ & $c_1$ & $100$ \\
  \hline
  $o_2$ & $c_2$ & $150$ \\
  \hline
  $o_3$ & $c_1$ & $120$ \\
  \hline
  $o_4$ & $c_1$ & $170$ \\
  \hline
  \end{tabular}
  \label{fig:sales-t1}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{price} & \# \\
  \hline
  $o_5$ & $c_2$ & $300$ & $+1$ \\
  \hline
  $o_6$ & $c_1$ & $150$ & $+1$ \\
  \hline
  $o_7$ & $c_2$ & $220$ & $+1$ \\
  \hline
  \end{tabular}
  \label{fig:sales-t2}
}
&
&
\\
&
\subfigure[]{
  \begin{tabular}{|c|c|c}
  \cline{1-2}
  \textit{o\_id} & \textit{cost} & \\
  \cline{1-2}
  $o_1$ & $10$ & $t_1$ \\
  \cline{1-2}
  $o_2$ & $20$ & $t_2$ \\
  \cline{1-2}
  $o_6$ & $15$ & $t_2$ \\
  \cline{1-2}
  \end{tabular}
  \label{fig:returns}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{o\_id} & \textit{cost} \\
  \hline
  $o_1$ & $10$ \\
  \hline
  \end{tabular}
  \label{fig:returns-t1}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cost} & \# \\
  \hline
  $o_2$ & $20$ & $+1$ \\
  \hline
  $o_6$ & $15$ & $+1$ \\
  \hline
  \end{tabular}
  \label{fig:returns-t2}
}
&
&
\\
\hdashline[2pt/2pt]
&
\subfigure[]{
  \begin{tabular}{|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{rev} \\
  \hline
  $o_1$ & $c_1$ & $-10$ \\
  \hline
  $o_2$ & $c_2$ & $-20$ \\
  \hline
  $o_3$ & $c_1$ & $120$ \\
  \hline
  $o_4$ & $c_1$ & $170$ \\
  \hline
  $o_5$ & $c_2$ & $300$ \\
  \hline
  $o_6$ & $c_1$ & $-15$ \\
  \hline
  $o_7$ & $c_2$ & $220$ \\
  \hline
  \end{tabular}
  \label{fig:sales-status-full}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{rev} \\
  \hline
  $o_1$ & $c_1$ & $-10$ \\
  \hline
  $o_2$ & $c_2$ & $150$ \\
  \hline
  $o_3$ & $c_1$ & $120$ \\
  \hline
  $o_4$ & $c_1$ & $170$ \\
  \hline
  \end{tabular}
  \label{fig:view-t1}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{rev} & \# \\
  \hline
  \cellcolor{lightgray}$o_2$ & \cellcolor{lightgray}$c_2$ & \cellcolor{lightgray}$150$ & \cellcolor{lightgray}$-1$ \\
  \hline
  $o_2$ & $c_2$ & $-20$ & $+1$ \\
  \hline
  $o_5$ & $c_2$ & $300$ & $+1$ \\
  \hline
  $o_6$ & $c_1$ & $-15$ & $+1$ \\
  \hline
  $o_7$ & $c_2$ & $220$ & $+1$ \\
  \hline
  \end{tabular}
  \label{fig:view-t2}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{rev} \\
  \hline
  $o_1$ & $c_1$ & $-10$ \\
  \hline
  \end{tabular}
  \label{fig:stream-t1}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|c|c|}
  \hline
  \textit{o\_id} & \textit{cat} & \textit{rev} & \# \\
  \hline
  $o_2$ & $c_2$ & $-20$ & $+1$ \\
  \hline
  $o_3$ & $c_1$ & $120$ & $+1$ \\
  \hline
  $o_4$ & $c_1$ & $170$ & $+1$ \\
  \hline
  $o_5$ & $c_2$ & $300$ & $+1$ \\
  \hline
  $o_6$ & $c_1$ & $-15$ & $+1$ \\
  \hline
  $o_7$ & $c_2$ & $220$ & $+1$ \\
  \hline
  \end{tabular}
  \label{fig:stream-t2}
}
\\
\hdashline[2pt/2pt]
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{cat} & \textit{gross} \\
  \hline
  $c_1$ & $265$ \\
  \hline
  $c_2$ & $500$ \\
  \hline
  \end{tabular}
  \label{fig:summary-full}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{cat} & \textit{gross} \\
  \hline
  $c_1$ & $280$ \\
  \hline
  $c_2$ & $150$ \\
  \hline
  \end{tabular}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{cat} & \textit{gross} \\
  \hline
  $c_1$ & $-15$ \\
  \hline
  $c_2$ & $+350$ \\
  \hline
  \end{tabular}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{cat} & \textit{gross} \\
  \hline
  $c_1$ & $-10$ \\
  \hline
  \end{tabular}
}
&
\subfigure[]{
  \begin{tabular}{|c|c|}
  \hline
  \textit{cat} & \textit{gross} \\
  \hline
  $c_1$ & $+275$ \\
  \hline
  $c_2$ & $+500$ \\
  \hline
  \end{tabular}
}
\\
& &
computation at $t_1$
&
computation at $t_2$
&
computation at $t_1$
&
computation at $t_2$
\\
&
batch execution
&
\multicolumn{2}{c;{2pt/2pt}}{view maintenance progressive execution}
&
\multicolumn{2}{c}{stream computing progressive execution}
\end{tabular}
\caption{(b)(e) Data arrival of \textit{sales} and \textit{returns} respectively;
(h)(m) expected \textit{sales\_status} and \textit{summary} at $t_2$;
(c)(f)(i)(n) and (d)(g)(j)(o) progressive execution of the view maintenance approach
at $t_1,t_2$ respectively;
(k)(p) and (l)(q) progressive execution of the stream computing approach at $t_1,t_2$ respectively.\kai{[This figure will be simplified as part of it is moved into Fig.~\ref{fig:tvr-basic}.]}}
\label{fig:all-tvr-ex}
\end{figure*}
\end{comment}

\section{From Section 4}

% To maintain $\gamma(S\leftouterjoin R)$, it materializes an update-independent
	% part $$M = \gamma_{\textit{o\_id};\textit{total}=\texttt{SUM}(\textit{cost})}(R)$$
	% When fed with the delta update to $S$, the delta to $\gamma(S\leftouterjoin R)$ can be computed by $$Q' =  \gamma_{\textit{category};\texttt{SUM}(r)}(\dt{S}{t_1}{t_2} \leftouterjoin \s{M}{t_1}),$$ where $r = \texttt{IF}(\textit{total} \texttt{ IS NULL}, \textit{price}, -\textit{total})$. $Q'$ computes the gross revenue per category by summing up the precomputed total cost in $M$ or the prices of the new orders added to $S$.
	% The auxiliary view $M$ can be further incrementally maintained by repeatedly
	% applying TVR-generating rules and the above inter-TVR equivalence rule
	% to generate higher-order views.

% \begin{figure*}[tb!]
% \centering
% \includegraphics[width=\textwidth]{figs/tvr-query-example.png}
% \caption{An example of TVR and TVR query}
% \label{fig:tvr-ex}
% \end{figure*}

% Applying a query on TVR's yields another TVR, formally defined as follows.
% In other words, the snapshot of TVR $Q(R)$ at $t$ is the same as
% applying $Q$ as a traditional relational query on the snapshot of $R$ at $t$.
% \begin{definition}
% Given TVR $R: T \rightarrow schema(R)$, applying a query $Q$ on $R$ defines another TVR
% on domain $T$, where $Q(R)$ is defined using its traditional relational semantics:
% $$Q(R)(t) = Q(R(t)), \forall t \in T$$
% \end{definition}
% As shown in Fig.~\ref{fig:tvr-ex}, $Q(R)(t_2)$, the snapshot of the TVR $Q(R)$ at $t_2$,
% is defined as if applying $Q$ directly $R$'s snapshot $R(t_2)$, yielding $\{(1, null), (2, 4)\}$.
% In the next section, we will show that the definition of $Q$ in
% different incremental computation models can be different,
% and thus leading to different snapshot definitions.

% \begin{enumerate}
% 	\item Run the SQL query at the triggering time points.
% 	\item Every time when the query is triggered, a snapshot of the TVR's at that time point
% 	is fed into the SQL query, and the SQL query simply executes as
% 	in traditional relational semantics, and deliver the query result as a snapshot.
% 	\item As time goes, the query results also vary over time, thus form a TVR.
% \end{enumerate}

% Trigger must be a subset of source TVR domain and the result TVR' domain
% $trigger \subseteq domain(TVR) \cap domain(TVR')$.
% Trigger determines the granularity that the query result TVR' changes.
% In other word, for any $t \in domain(TVR') - trigger$, the query semantics is defined as
% $snapshot(TVR', t) = snapshot(TVR', floor(t))$
% where $floor(t) = max\{t'|t' \in trigger, t' < t\}$.
% It means that

% Traditional data warehouses answer query $Q$ at the triggering time,
% when data is fully collected and fixed (e.g., $t_3$ in Fig.~\ref{fig:tvr-ex}),
% by computing $Q$ on the final snapshot of the TVR $R(t_3)$,
% yielding the query result $\{ (2, 4) \}$.
% On the contrary, computing $Q$ in a progressive way,
% similar to the approach taken by stream computing or view maintenance work,
% can execute $Q$ earlier than $t_3$, e.g., at $t_1$ and $t_2$
% in a way not on the snapshot directly.

% The essence of ideas behind incremental computation is to view the changes of a TVR
% from a different perspective than snapshot, that is, through a delta perspective.
% We denote the difference between two snapshots of TVR $R$ at $t, t' \in T$ ($t < t'$)
% as the \emph{delta} of $R$ from $t$ to $t'$, denoted $\dt{R}{t}{t'}$.
% \kai{As discussed in~\cite{partial}, the difference between snapshots
% can take forms of missing tuples, phantom tuples,
% or incorrect values, or even mixes of the above.}
% As we will discuss later, deltas can have different forms under different incremental models,
% but in general consists of two types of \emph{operations}:
% positive ($+$) and negative ($-$).
% $+$ represents changes like insertion, adding a value, etc.,
% while $-$ represents those like deletion, subtracting a value, etc.
% Formally,
% \begin{definition}
% $\dt{R}{t}{t'}$ defines a mapping from a time interval ($T^2$) to a bag of tuples
% belong to schema $schema(R) \times \{+,-\}$, such that
% $$R(t) \oplus \dt{R}{t}{t'} = R(t')$$
% where $\oplus$ is a merge operator defined on $R(t)$ and $\dt{R}{t}{t'}$.
% \end{definition}
% % By repeatedly applying the above rule, we can extend to:
% % $$R(t_n) = R(t_0) \oplus [\bigoplus_{t_i \in T, 0 \leq i < n}{\Delta R(t_i, t_{i+1})}]$$
% Sometimes, one can easily define the inverse operator of $\oplus$, denoted $\ominus$,
% and we have
% $$\dt{R}{t}{t'} = R(t') \ominus R(t)$$
% E.g., $\Delta R(t_2, t_3) = \{(1, 100, null, -), (1, 300, 5, +)\}$;
% merging it with $R(t_2)$ deletes $-$ tuples $(1, 100, null)$
% and inserts $+$ tuples $(1, 300, 5)$, yielding $R(t_3)$.
% And instead of computing $Q(R)(t_2) and Q(R)(t_3)$ directly,
% we compute a delta query on $\Delta R(t_1, t_2)$ and $\Delta R(t_2, t_3)$,
% and merge the results $(2, 4, +)$ and $(1, null, -)$ with $Q(R)(t_1)$ to get $Q(R)(t_3)$.

% Although incremental computation has been extensively studied and
% have many different techniques under different applications
% such as view maintenance and streaming computing,
% With the above definitions, the key idea behind incremental computation
% can be concisely summarized as seeking for
% \textbf{using computation on deltas to achieve the same result as computation on snapshots}, i.e.,
% $$Q(R(t')) = Q(R(t) \oplus \Delta R (t, t')) = Q(R(t)) \oplus \Delta Q(R(t), \dt{R}{t}{t'})$$

% Actually, the stream computing method, the view maintenance method,
% and any other delta computation method rely on the same set of delta computation rules.
% Furthermore, these TVR rules live well with all the existing relational algebra rewritings.
% E.g., the same filter push down optimization can be applied no matter
% the tree is a snapshot query, or a delta query, or a mix of both.

% We can see that existing approaches define new incremental computation models
% through the following process:
% \begin{itemize}
% \item Model-Defining Rule. As shown by Observation~\ref{obs:diff-model},
% given a query $Q$, users may compute a different query $Q'$ than $Q$,
% this is usually defined in the form of a set of rules that map
% (possibly a subset of) relational algebra operators to a different set of algebra operators.
% We denote this set of rules as $r^{def}$.

% \item Model Delta Rule. Within a fixed incremental model, the delta computation method
% serves as the core. As shown in Observation~\ref{obs:diff-delta}, delta computation
% is defined by a set of equivalent rewritings on snapshots and deltas, and the merge operator
% between snapshots and deltas, e.g., Eq.~\ref{eq:delta}.
% We denote this set of rules as $r^{delta}$.

% \item Model Conversion Rule. To convert an intermediate results delivered by an incremental
% model to the target final result, or to explore the possible incremental plan space by
% combining different incremental models, one an add equivalent rewritings between snapshots
% of different TVR's, e.g., Eq.~\ref{eq:conv}. We denote this set of rules as $r^{conv}$.
% \end{itemize}
% We can see that an incremental computation model is defined by
% a triple $(Q, \Delta Q, +)$:
% (1) the query semantics $Q$ defined on snapshots;
% (2) the incremental query semantics $\Delta Q$ defined on deltas and snapshots;
% (3) the \emph{merge} operator $+$ used to combine snapshot and delta.
% % Furthermore, snapshot and delta are two sides of the TVR coin and can transform to each other,
% % e.g.,
% % (1) snapshots can be \emph{merged} with deltas
% % to construct new snapshots, and (2) deltas can be constructed
% % through taking difference between snapshots,
% % providing the flexibility in searching for optimal plans during query optimization.
% Furthermore, different incremental computation models can transform to each other,
% providing a way to unify different incremental models.
% In summary, our progressive computation framework,
% \emph{a general framework that allows plugging in various incremental computation techniques,
% and enabling automatic cost-based search for optimal plans},
% allow users to plug in different incremental computation models
% by providing a triple $(r^{def}, r^{delta}, r^{conv})$.
% In the next section, we demonstrate how we can define
% the above discussed view maintenance and stream computing approaches
% on our framework,
% Following from this observation, our progressive incremental framework
% allows users to plug in different incremental computation models
% following the above process,
% by letting them specifying the above three main elements,
% and enables cost-based optimization among all possible incremental plans.
% Thanks to the strong compositionality
% of the relational algebra, $Q$ and $\Delta Q$ can be defined using
% delta rules for individual relational operators.
% Next, we show how we integrate three commonly used incremental computation models.

% The above example reveals two access methods to a TVR: \emph{snapshot} and \emph{delta}:

% Informally, snapshot accesses the definition of a TVR---the bag of tuples
% that it represents---at a specific time, or denoted in a function form $snapshot(R, t)$
% where $t$ is a time point from $R$'s time domain.
% Usually, the semantics of a query on TVR is naturally defined by its snapshot.
% That is, for a TVR $R'$ defined by another TVR $R$ as $R' = Q(R)$, $R'$ can be
% naturally defined through its snapshot---at any time $t$,
% $snapshot(R', t) = Q(snapshot(R, t))$.

% The snapshot form is one perspective to observe how a TVR changes over time.
% Another perspective is through delta. Delta can be derived from snapshot:
% delta accesses the difference between the snapshots of relation $R$ at $t_1$ and $t_2$,
% or in a functional way $delta(R, t_1, t_2)$ where $t_1, t_2 \in T, t_1 < t_2$.

% The definition shows that snapshot and delta are deeply connected
% and can transform to each other:
% \begin{enumerate}
% 	\item $delta(R, t_1, t_2)$ can be constructed through taking difference between
% 	$snapshot(R, t_2)$ and $snapshot(R, t_1)$.
% 	\item $snapshot(R, t_1)$ can be \emph{merged} with $delta(TVR, t_1, t_2)$
% 	to construct $snapshot(TVR, t_2)$.
% \end{enumerate}
% Given the delta history, we could reconstruct the snapshot history at any time;
% given the snapshots history, we could also reconstruct the delta history.
% All possible timestamps of the snapshots or deltas constitute the time domain $T$ of the TVR. In this case, the time domain $T$ is $\{t1, t2, t3, t4\}$. t could be of actual Datetime type, it could as well be a logical timestamp.

% The time domain $T$ doesn't necessarily captures all the changes of the TVR.
% For example, if we take hourly snapshot starting $1$pm and ending $4$pm,
% we don't know what the snapshot looks like at $1$:$30$.
% This is the granularity of the TVR, and it could be very fine grained
% (snapshot when every tuple changes), or very coarse grained (snapshot every hour).
% The same granularity also applies to delta form,
% the delta update tuples at $2$pm means the cumulative changes
% from the previous update ($1$pm) to now.

% The above observation gives us a good sense of snapshot and delta as different ways to access
% a TVR, and their relationship.
% This general intuition actually lays a good step stone towards our progressive relational model.
% However, we note that here we avoid giving a formal definition of
% snapshot and delta on purpose, as we will show next that snapshot and delta can be have
% different variations, and need much more sophisticated analysis.


\begin{comment}

\subsection{Progressive Computation Framework}

In this section, we demonstrate how to integrate into our framework
four incremental models:
retractable/non-retractable bag models,
and retractable/non-retractable value models.
And we will show that previously discussed view maintenance
and stream computing incremental models are special subspaces
in the possible incremental plan space enabled by these four incremental models.

% \noindent
% \textbf{Formal Definitions}.
% We borrow the CQL paper~\cite{cql}, and model a relation varying with time
% using the concept of a \emph{Time-Varying Relation} (TVR).
% Formally,
% \begin{definition}
% A time-varying relation $R$ is a mapping from a time domain $T$ to a bag of tuples
% belonging to the schema of R.
% \end{definition}
% A \emph{snapshot} of $R$ defines the bag of tuples of $R$ at time $t \in T$, denoted $R(t)$.
% $R(t)$ is just a traditional relation.

% Applying a query on TVR's yields another TVR, formally defined as follows.
% In other words, the snapshot of TVR $Q(R)$ at $t$ is the same as
% applying $Q$ as a traditional relational query on the snapshot of $R$ at $t$.
% \begin{definition}
% Given TVR $R: T \rightarrow schema(R)$, applying a query $Q$ on $R$ defines another TVR
% on domain $T$, where $Q(R)$ is defined using its traditional relational semantics:
% $$Q(R)(t) = Q(R(t)), \forall t \in T$$
% \end{definition}
% % \begin{enumerate}
% % 	\item Run the SQL query at the triggering time points.
% % 	\item Every time when the query is triggered, a snapshot of the TVR's at that time point
% % 	is fed into the SQL query, and the SQL query simply executes as
% % 	in traditional relational semantics, and deliver the query result as a snapshot.
% % 	\item As time goes, the query results also vary over time, thus form a TVR.
% % \end{enumerate}

% % Trigger must be a subset of source TVR domain and the result TVR' domain
% % $trigger \subseteq domain(TVR) \cap domain(TVR')$.
% % Trigger determines the granularity that the query result TVR' changes.
% % In other word, for any $t \in domain(TVR') - trigger$, the query semantics is defined as
% % $snapshot(TVR', t) = snapshot(TVR', floor(t))$
% % where $floor(t) = max\{t'|t' \in trigger, t' < t\}$.
% % It means that

% The essence of incremental computation is to view the changes of a TVR from
% a different perspective than snapshot, that is, through a delta perspective.
% We denote the difference between two snapshots of TVR $R$ at $t, t' \in T$ ($t < t'$)
% as the \emph{delta} of $R$ from $t$ to $t'$, denoted $\dt{R}{t}{t'}$.
% As we will discuss later, deltas can have different forms under different incremental models,
% but in general can be classified into two \emph{operations}:
% positive ($+$) and negative ($-$).
% $+$ represents changes like insertion, adding a value, etc.,
% while $-$ represents those like deletion, subtracting a value, etc.
% Formally,
% \begin{definition}
% $\dt{R}{t}{t'}$ defines a mapping from a time interval ($T^2$) to a bag of tuples
% belong to schema $schema(R) \times \{+,-\}$, such that
% $$R(t) \oplus \dt{R}{t}{t'} = R(t')$$
% where $\oplus$ is a merge operator defined on $R(t)$ and $\dt{R}{t}{t'}$.
% \end{definition}
% % By repeatedly applying the above rule, we can extend to:
% % $$R(t_n) = R(t_0) \oplus [\bigoplus_{t_i \in T, 0 \leq i < n}{\Delta R(t_i, t_{i+1})}]$$
% Sometimes, one can easily define the inverse operator of $\oplus$, denoted $\ominus$,
% and we have
% $$\dt{R}{t}{t'} = R(t') \ominus R(t)$$

% Although incremental computation has been extensively studied and
% have many different techniques under different applications
% such as view maintenance and streaming computing,
% With the above definitions, the key idea behind incremental computation
% can be concisely summarized as seeking for
% \textbf{using computation on deltas to achieve the same result as computation on snapshots}, i.e.,
% $$Q(R(t')) = Q(R(t) \oplus \Delta R (t, t')) = Q(R(t)) \oplus \Delta Q(R(t), \dt{R}{t}{t'})$$
% We can see that an incremental computation model is defined by a triple $(Q, \Delta Q, \oplus)$:
% (1) the query semantics $Q$ defined on snapshots;
% (2) the incremental query semantics $\Delta Q$ defined on deltas and snapshots;
% (3) the \emph{merge} operation $\oplus$ used to combine snapshot and delta.

% Following from this observation, our progressive incremental framework
% allows users to plug in incremental computation techniques by letting them
% specifying the above three main elements. Thanks to the strong compositionality
% of the relational algebra, $Q$ and $\Delta Q$ can be defined using
% delta rules for individual relational operators.
% Next, we show how we integrate three commonly used incremental computation models.

\noindent
\textbf{Retractable Bag Model}.
The incremental bag semantics is arguably the most simple incremental computation model.
We use the bag semantics to model the snapshots and deltas of a TVR,
as it is the most commonly adopted model in commercial RDBMSs.
In the bag semantics, for a TVR $R$, $R(t)$ and $\dt{R}{t}{t'}$
are all functions mapping from the schema of $R$ to an integer, named multiplicity.
Where the multiplicity represents the number of occurrences of a tuple
in the relation. Specifically, for $\dt{R}{t}{t'}$, a positive multiplicity represents
insertion of a tuple, whereas a negative multiplicity represents deletion.
Updates are modeled as insertions followed by deletions.
Following this definition, the merge operator $+$ is defined as additive union
of bag relations, summing up multiplicities of corresponding tuples together.
Furthermore, $+$ has an inverse operator $-$ defined as subtractions
of multiplicities, so that we have $R(t') - R(t) = \dt{R}{t}{t'}$.
$\Delta Q$ is defined using the following rules~\cite{dupView}.
Note that we do not have an efficient delta rule for aggregate.
% In the following, for simplicity, we omit the time parameter of snapshot and delta
% if it will not incur confusion.

\begin{itemize}
	\item \texttt{SELECT}: $\sigma_\theta (R(t) + \dt{R}{t}{t'}) = \sigma_\theta(R(t)) + \sigma_\theta(\dt{R}{t}{t'})$
	\item \texttt{PROJECT}: $\pi_{\bar{A}}(R(t) + \dt{R}{t}{t'}) = \pi_{\bar{A}}(R(t)) + \pi_{\bar{A}} (\dt{R}{t}{t'})$
	\item \texttt{JOIN}:
	$[R_1(t) + \Delta R_1(t, t')] \bowtie [R_2(t) + \Delta R_2(t, t')] = [R_1(t) \bowtie R_2(t)] + [\Delta R_1(t, t') \bowtie R_2(t)] + [R_1(t) \bowtie \Delta R_2(t, t')] + [\Delta R_1(t, t') \bowtie \Delta R_2(t, t')]$
	\item \texttt{UNION}: $[R_1(t) + \Delta R_1(t, t')] \cup [R_2(t) + \Delta R_2(t, t')] = [R_1(t) \cup R_2(t)] + \Delta R_1(t, t') + \Delta R_2(t, t')$
	\item \texttt{DIFFERENCE}:
	$$(R_1 + \Delta R_2) - (R_2 + \Delta R_2) = (R_1 - R_2) + (\Delta R_1 - R_2 - \Delta R_2) - \Delta R_2$$
	% \item \texttt{AGGREGATE}\footnotemark: $\Delta \gamma_{\bar{A},\Psi=sum} R = \gamma_{\bar{A},\Psi=sum}(\Delta R)$\footnotetext{
	% $\gamma_{\bar{A},\Psi}$ represents an \texttt{AGGREGATE} operator
	% with group-by column $\bar{A}$ and aggregate function $\Psi$.}
\end{itemize}

\noindent
\textbf{Non-retractable Bag Model}.
Append-only incremental bag semantics are the most commonly used model in
traditional streaming processing. Different from the incremental bag semantics,
it does not allow retraction of tuples, i.e., deletion of outputted tuples.
The append-only incremental bag semantics uses the same definition of snapshot,
delta and the merge operator $+$ as the incremental bag semantics,
except that it is only defined on positive relational algebra (excluding set difference)..
% \begin{itemize}
% 	\item \texttt{DIFFERENCE}:
% 	$(R_1 \oplus \Delta R_2) - R_2 = (R_1 - R_2) \oplus \Delta R_1$; whereas
% 	$R_1 - (R_2 \oplus \Delta R_2)$ will not output.

% 	\item \texttt{AGGREGATE}: If $\Delta R$ exists, aggregate will not output results;
% 	otherwise, aggregate will output $\gamma_{\bar{A},\Psi=sum} R$.
% \end{itemize}

\kai{[up to here]}

\begin{wip}

\noindent
\textbf{Generalized Incremental Bag Semantics}.
The most common delta is defined on a set - an \emph{insertion} delta means inserting a tuple into a set and a \emph{deletion} delta means deleting a tuple from a set.
There's another rather special kind of \emph{value} delta that could enable a lot more optimization opportunities.
The \emph{value} delta is normally a result of an aggregation.
Next, we'll use an example to illustrate the difference.
Consider a relation $R$ with schema (order\_id: string, category: string, amount: double)
with the initial data as in Fig.~\ref{fig:init-val}.
We would like to compute the total amount per category
on $R$, and get the aggregate result as in Fig.~\ref{fig:init-aggr}.

\begin{figure*}[htb!]
\centering
\begin{tabular}{cccc}
\subfigure[]{
	\begin{tabular}{|c|c|c|}
		\hline
		order id & category & amount \\
		\hline
		1 & food & 150 \\
		\hline
		2 & cloth &100 \\
		\hline
	\end{tabular}
	\label{fig:init-val}
} &
\subfigure[]{
	\begin{tabular}{|c|c|}
		\hline
		category & amount \\
		\hline
		food & 150 \\
		\hline
		cloth &100 \\
		\hline
	\end{tabular}
	\label{fig:init-aggr}
} &
\subfigure[]{
	\begin{tabular}{|c|c|}
		\hline
		category & amount \\
		\hline
		food & 150 \\
		\hline
		cloth & 300 \\
		\hline
	\end{tabular}
	\label{fig:new-aggr}
} &
\subfigure[]{
	\begin{tabular}{|c|c|}
		\hline
		TS & Delta Operation \\
		\hline
		t3 & DELETE (cloth, 100) \\
		\hline
		t3 & INSERT (cloth, 300) \\
		\hline
	\end{tabular}
	\label{fig:delta}
}
\end{tabular}
\caption{(a) Initial data of $R$, (b) initial aggregation result,
(c) new aggregation result, and (d) the delta}
\end{figure*}

If we use the incremental bag semantics delta, given a delta change to source table T:
\emph{t3, INSERT (3, cloth, 200)}.
The new aggregation result and the delta value are shown in
Fig.~\ref{fig:new-aggr} and~\ref{fig:delta}.
We could possibly compute the new aggregation result by:
Compute the new snapshot of source table T, and re-compute the new aggregation result.
This process could incur lots of overhead.
Instead we could also try combining previous snapshot and new delta method:
\begin{itemize}
	\setlength{\itemsep}{0pt}
	\setlength{\parsep}{0pt}
	\setlength{\parskip}{0pt}
	\item load previous result from disk (food, 150), (cloth, 100)
	\item use JOIN to find tuples to update, output negative delta: DELETE (cloth, 100)
	\item compute aggregation again to output the new delta, e.g., (cloth, 100) and (cloth, 200) can be regarded as INSERT (cloth, 300)
\end{itemize}

This method seems feasible, however, if there's another change to source table T:
\emph{t4, DELETE (1, food, 150)}.

Load previous result from disk: (food, 150), (cloth, 300)
Find and output negative delta: \emph{DELETE (food, 150)}.
And then compute aggregation again: (food, 150), -(food, 150) to ???

There's no way we could know whether the \emph{food} group still exists or not.
If we output (food, 0), then the result would be incorrect.
If we don't output, it's still incorrect because there could exist a tuple with amount 0.

For aggregation operators, the \emph{set} delta cannot help us at all. We are forced to fall back to using all snapshots.
The \emph{set} delta values means \emph{adding a tuple to the set} or \emph{deleting a tuple from the set}. In the case of aggregation, we rather want something to represent \emph{changing an aggregation value of an existing tuple}.

Given a delta change to source table T:
 \emph{t3, INSERT (3, cloth, 200)}

We now output a new kind of delta: \\
 \centerline{\emph{t3, (cloth, +200), }}
 \centerline{\emph{with (SUM() function on aggregated column total amount)}}
It represents the change of the \emph{value} of the \emph{total\_amount} column.

When combining the new \emph{value} delta with an existing snapshot to produce new snapshot,
instead of doing union/set diff to apply positive/negative delta,
we do:
\begin{enumerate}
	\setlength{\itemsep}{0pt}
	\setlength{\parsep}{0pt}
	\setlength{\parskip}{0pt}
	\item [1)] find the existing tuple of same group by key: (cloth, 100)
	\item [2)] apply the aggregation function to produce a new tuple: SUM(100, +200) to (cloth, 300).
\end{enumerate}

If we only want the aggregation delta result, we can simply output the \emph{value} delta,
without loading the previous aggregation result.

However, having the \emph{value} delta on aggregation column alone won't solve the deletion problem.

We need another column: \emph{total count}, indicating the number of tuples producing this aggregation result.
Furthermore, the \emph{delta operation} column is generalized as the \emph{multiplicity} column.
\emph{Multiplicity} means \#(number) of tuples, adding a tuple means +1, deleting a tuple means -1.

With the initial table T value:
\begin{table}[ht!]
	\centering
	\begin{tabular}{|c|c|c|}
		\hline
		order\_id & category & amount \\
		\hline
		1 & food & 150 \\
		\hline
		2 & cloth &100 \\
		\hline
	\end{tabular}
\end{table}

We instead store the following aggregation result as state:

\begin{table}[ht!]
	\centering
	\begin{tabular}{|c|c|c|}
		\hline
		category & total\_amount & total\_count \\
		\hline
		food & 150 & 1 \\
		\hline
		cloth &100 & 1 \\
		\hline
	\end{tabular}
\end{table}

With the delta change: \emph{t3, INSERT (3, cloth, 200)}
We have the new delta: \emph{t3, (cloth, +200, +1)}
Applying the aggregation function to produce new snapshot:

\begin{table}[ht!]
	\centering
	\begin{tabular}{|c|c|c|}
		\hline
		category & total\_amount & total\_count \\
		\hline
		food & 150 & 1 \\
		\hline
		cloth &300 & 2 \\
		\hline
	\end{tabular}
\end{table}


With the delta change: \emph{t4, DELETE (1, food, 150)}
We have the new delta: \emph{t4, (food, -150, -1)}

Applying the aggregation function to produce new snapshot:

\begin{table}[ht!]
	\centering
	\begin{tabular}{|c|c|c|}
		\hline
		category & total\_amount & total\_count \\
		\hline
		food & 0 & 0 \\
		\hline
		cloth &300 & 2 \\
		\hline
	\end{tabular}
\end{table}

In this way, a total count of 0 clearly means there's no tuple with category \emph{food}.
Multiplicity operates in the same way as \emph{value} delta - the delta updates are applied to the value of multiplicity column.

We use a generalized bag semantics that generalizes bag relations to tuple multiplicities
that can be arbitrary aggregate functions.
Accordingly, the merge operators are also extended to be also applied on aggregate functions.

\begin{itemize}
	\item \texttt{SELECT}: $\sigma_\theta (R \oplus \Delta R) = \sigma_\theta(R) \oplus \sigma_\theta(\Delta R)$
	\item \texttt{PROJECT}: $\pi_{\bar{A}}(R \oplus \Delta R) = \pi_{\bar{A}}(R) \oplus \pi_{\bar{A}} (\Delta R)$
	\item \texttt{JOIN}:
	$(R_1 \oplus \Delta R_1) \bowtie (R_2 \oplus \Delta R_2) = (R_1 \bowtie R_2) \oplus (\Delta R_1 \bowtie R_2) \oplus (R_1 \bowtie \Delta R_2) \oplus (\Delta R_1 \bowtie \Delta R_2)$
	\item \texttt{UNION}: $(R_1 \oplus \Delta R_1) \cup (R_2 \oplus \Delta R_2) = (R_1 \cup R_2) \oplus (\Delta R_1) \oplus (\Delta R_2)$
	\item \texttt{DIFFERENCE}:
	$$(R_1 \oplus \Delta R_2) - R_2 = (R_1 - R_2) \oplus \Delta R_1$$
	$$R_1 - (R_2 \oplus \Delta R_2) = (R_1 - R_2) \oplus \Delta R_1 - \Delta R_2 ?$$

	\item \texttt{AGGREGATE}: $\Delta \gamma_{\bar{A},\Psi=sum} R = \gamma_{\bar{A},\Psi=sum}(\Delta R)$
\end{itemize}

Multiplicity could be generalized to our normal \emph{set} delta as a special column to replace delta operation: INSERT as +1, DELETE as -1 . In this way, we have a uniform representation of delta values:
Suppose the delta schema S include columns A\_1, A\_2, ... A\_n,
We can mark each column as either a \emph{fixed} column or \emph{aggregated value} column.

\begin{table}[ht!]
	\centering
	\begin{tabular}{|c|c|c|c|c|c|c|c|}
		\hline
		A\_1 & A\_2 & \dots & A\_k & \dots & A\_n & \# & TS \\
		\hline
		fixed & fixed & \dots & $\oplus$ & \dots & fixed & $\pm 1$ & t \\
		\hline
	\end{tabular}
\end{table}

For each \emph{aggregated value} column, the aggregation function must be marked.
There are two special columns that must exist: \#(multiplicity) and ts(timestamp).
Some fixed columns can be specified as \emph{key}, if none is specified, then all fixed columns will be used.
The \emph{key} could be inferred by the system in some cases,
for example, the group by columns will become the key after aggregation.

\noindent
\textbf{Relationship between Different Semantics}.

\end{wip}

\end{comment}


% \kai{[Note that inputs are not relational operators. Therefore, supposedly
% TVR rewriting rules, especially TVR-generating rules, do not expand inputs
% along the time line. Think about it, how can you define a rule that knows
% what a relation look like at a specific time?
% That is why in the example above, we say Group 3-Group 6 is generated by
% "seeding the snapshots and deltas of the input relations",
% instead of applying TVR-generating rules.
% In short, issues like that incurred by expanding a time-specific empty input into TVR
% are implementation issues, not theoretical issues.
% That is why we do not need to discuss the following.]}
% \noindent
% \textbf{Interaction between TVR/Traditional Rewriting Rules}.
% Generally, traditional SQL rewriting rules can work well with TVR rewriting rules
% without modification. For instance, in the example Memo shown in Fig.~\ref{fig:memo},
% traditional rules such as a hash-based implementation of inner join
% can be simply applied to Group 7 and Group 8.
% However, there are cases we need to pay special attentions to.
% Relational algebra is data-independent.
% The logic of relational operators are only determined by their defining properties,
% independent of their input data.
% By leveraging this data-independence, SQL rewriting rules are mostly data-independent too.
% As an example, consider a filter-pushdown rule that pushes a filter operator
% below a project operator.
% This rule can be applied as long as the filter condition
% can be evaluated on the input schema of the project operator,
% despite the content of the project operator's input.
% But there are rules that are data-dependent. An example is that \kai{something}.
% Data dependent rules can generate data dependent patterns.
% Within each logical equivalence class, each operator is tagged with an indicator
% whether it is time-specific or not.
% Rules applied on time-specific patterns will generates patterns that are time-specific
% too.
% TVR rewriting rules cannot match with operators that are time-specific.
% Note that by default we can mark all traditional rewriting rules as time-specific.
% This will not affect the correctness of the exploration,
% as all patterns will eventually be explored. \kai{why?}
% It will also affect the efficiency a bit, see the subsection below.
% Based on the above observation, we classify the rules into
% data-independent and data-dependent ones,
% and reduce redundancy for data-independent rules during query optimization.
% Formally, we define \emph{data-independent properties} as properties that do not change
% with data.
% Examples of such properties are the schema of the input and output,
% the distribution of a physical implementation, the primary/foreign key of a relation, etc.;
% whereas examples of data-dependent properties include number of rows in the input data, etc.
% We define \emph{data-independent rules} as the rules implemented only referencing
% data-independent properties.
% \sys{} provides APIs for an optimizer developer to specify which rules are data-independent.


% Abstract Converters.



\begin{comment}

\noindent
\textbf{Batch Application of Data-Independent Rules}.
Relational algebra is data-independent.
The logic of relational operators are only determined by their defining properties,
independent of their input data.
By leveraging this data-independence, SQL rewriting rules are mostly data-independent too.
Rules can be applied to generate all viable plan alternatives no matter of the input data,
and rely the optimizer to cost all plan alternatives based on the concrete input data
to find the optimal plan (we will discuss plan costing in \S\ref{sec:select-a-plan}).
As an example, consider a filter-pushdown rule that pushes a filter operator
below a project operator.
This rule can be applied as long as the filter condition
can be evaluated on the input schema of the project operator,
despite the content of the project operator's input.
On the other hand, a Memo contains many data-independent similarities along the time dimension.
To give you an idea, in Fig.~\ref{fig:memo}, the inner join in Group 7 and Group 8
are exactly the same, i.e., having the same join condition etc.,
modulo the input data they scanned at different time.
However, with a naive implementation, rules such as a hash-based implementation of
inner join have to be repeated applied on both Group 7 and Group 8,
incurring many redundancies.

TVR twin snapshots: if one is a base relation, then they are twins if they are snapshots of the same TVR; if one is a relational operator, then they are twins if their inputs are TVR twins,
they have the same data-independent properties, and they are snapshots of the same TVR.
TVR twin deltas:

Based on the above observation, we classify the rules into
data-independent and data-dependent ones,
and reduce redundancy for data-independent rules during query optimization.
Formally, we define \emph{data-independent properties} as properties that do not change
with data.
Examples of such properties are the schema of the input and output,
the distribution of a physical implementation, the primary/foreign key of a relation, etc.;
whereas examples of data-dependent properties include number of rows in the input data, etc.
We define \emph{data-independent rules} as the rules implemented only referencing
data-independent properties.
\sys{} provides APIs for an optimizer developer to specify which rules are data-independent.
As the snapshots (deltas) of the same TVR are of the same data-independent
properties, we are in particular interested in patterns that are the same except with different input data, where the input data are snapshots(deltas) of the same TVR.
We refer to these patterns as \emph{TVR-twin patterns}.
E.g., the trees rooted at the inner join in Group 7 and Group 8 are TVR-twin patterns.
The basic idea is that if a data-independent rule matches a pattern $P$,
it should match all TVR-twin patterns of $P$,
and the generated patterns are TVR-twin patterns of that generated from $P$.
The optimization process is carried out in four phases:
\begin{enumerate}[nosep,leftmargin=*]
\item We seed the Memo with different inputs $I$ covering a pre-defined set of
snapshots and/or deltas of their TVR's.
We discuss how to determine the set of snapshots and deltas in \S\ref{sec:opt}.

\item \kai{We pick a subset of inputs $I_0$, usually covering the snapshots of two time points
and the deltas between them,
and apply data-independent rules on this subset of Memo.}

\item \kai{We copy the above Memo by substituting inputs in $I_0$ with inputs in $I-I_0$.
the tree with different leaves (inputs).
During the copy process, every time we add new nodes and relationships into the Memo, we deduplicate
the matched rule patterns. If we are sure the rule has been fired before in the seed time frame,
we skip it. We also provide APIs for users to completely disable some rules in this Phase in order to save the match time too.}

\item \kai{We continue with the optimization of the rule engine as is.}
\end{enumerate}

% We introduce a compression scheme that can merge the above shown duplicates and reduce
% the number of rule applications. In the Memo, algebra expressions are represented with
% time-agnostic operator nodes whenever possible, with kleene star on the time point.
% The time-specific operator nodes can be instantiated from these time-agnostic operator
% with a function createInstance(time).
% The Memo needs to record the time-specific operator in order to keep track of
% the best plan of each subtree at each specific time. However, this recording
% is done without instantiating the time-specific operator, instead, we record
% the time-agnostic operator along with the time argument needed to instantiate the
% time-specific node.
% The time-specific operator are only instantiated needed, specifically at the time
% constructing the optimal plan.

% For rules that are time agnostic. It can be applied directly on the time-agnostic expression
% tree. Only time-sensitive rules, e.g., the rule that finds a table scan at a specific time
% is an empty relations, work on time-specific expressions and these expressions are kept in
% the Memo alongside the time-agnostic ones.

% \kai{[We have to discuss how we can represent algebra expressions generated by TVR rules,
% as these rules usually require a specific relationship between different TVR forms, e.g.,
% when merge previous snapshot with a delta, the time intervals covered by them must be
% consecutive]}

\end{comment}


\begin{comment}
\subsection{Exploiting Progressive Properties}

% Traditional optimizers identified a set of properties,
% such as data distribution and collation, useful to cost-based optimization.
% These properties can affect the applicability of transformations and
% thus affect the optimal plan chosen.
In this section, we identify a list of properties that if exploited
during progressive planning, could lead to better execution plans.

\noindent
\textbf{Delta Result Properties}.
Progressive execution produces partial results.
As discussed in \S\ref{sec:concept}, deltas produced by progressive execution
can have two types of properties:
(1) from a multiplicity perspective, the delta can either add tuples or delete tuples
or both;
(2) from a value perspective, the delta can be either positive or negative or both.
These properties can directly affect the incremental methods applicable.
% partial results can have
% Compared to the \emph{true} result that would be produced on the complete data,
% Partial results can differ in two properties: cardinality and correctness~\cite{partial}.
% Specifically, from the cardinality aspect, a partial result may miss some tuples,
% or have extra tuples, or even both relative to the true result;
% from the correctness aspect, a partial result may have incorrect data values
% compared to the true result.
Consider Example~\ref{ex:partial-property} that finds high-revenue categories.
% Assume \texttt{sales} is append-only.
Without extra information, we can only conclude that
% If we simply conclude that as \texttt{sales} is incomplete and thus
as \texttt{SUM}(\textit{price}) may be updated,
deltas to \textit{res} may both insert and delete tuples.
However, if we know that \textit{price} is always positive and \textit{sales} is append-only,
then \texttt{SUM}(\textit{price}) is strictly increasing.
We can conclude that deltas of \textit{res} are append-only too.
This can further affect the downstream queries of \textit{res},
e.g., whether the stream computing approach is applicable for incremental computation.
\begin{example}[High-Revenue Categories]
\begin{alltt}
\small
\textit{res} = SELECT \textit{category} FROM \textit{sales}
       GROUP BY \textit{category}
       HAVING SUM(\textit{price}) > 1000,000;
\end{alltt}
\label{ex:partial-property}
\end{example}

\noindent
\textbf{Temporal Ordering Property}.
Progressive execution introduces the temporal dimension into query execution.
Therefore, knowing the temporal ordering of data will tell us useful information
about how delta updates could look like, which in turn affect the inference of partial result
properties and further the query optimization.
To illustrate, consider the \textit{sales\_status} query in Example~\ref{ex:pipeline}.
If we know \textit{o\_id} is a self-increment identifier,
and find that the max \textit{o\_id} in \textit{returns}
is already greater than or equal to the max in \texttt{sales},
we can infer that any tuple in \textit{sales} that cannot join with \textit{returns}
will never join in the future,
and thus deltas of \textit{sales\_status} are append-only and
will not cause retraction overhead.

\noindent
\textbf{Primary/foreign Key Properties}.
Although commonly utilized in traditional optimizers,
primary/foreign key properties have interesting interactions with progressive execution.
Many incremental computation methods have special optimizations
in the case of primary/foreign key constraints.
Taking the outer join view maintenance~\cite{outerjoin-view} as an example,
the computation of deltas of $Q^D$ and $Q^I$ can be simplified for foreign key joins.
% Specifically, primary/foreign key constraints indicate uniqueness of tuples
% in both snapshot and delta relations.
% Again, consider incremental computation of the outer join
% in query \texttt{ext\_sales} in Example~\ref{ex:running}.
% Consider we delete the tuple $p_1$ from \texttt{promotions}.
% Without knowing \texttt{promo\_no} is the primary key of \texttt{promotions}, i.e.,
% the outer join is a foreign key join, we are not sure that if this deletion
% may generate a new tuple $\{o_1, 100, null\}$ in \texttt{ext\_sales}.
% This is because that if there are still other tuples with \texttt{promo\_no}$=p_1$
% in \texttt{promotions}, tuple $o_1$ still can join with them.
% On the contrary, if we know that \texttt{promo\_no} is the primary key of \texttt{promotions},
% then deleting tuple $p_1$ from \texttt{promotions} will for sure generate
% $\{o_1, 100, null\}$ in \texttt{ext\_sales}, since there must not be another tuple
% in \texttt{promotions} with the same primary key $p_1$.
\end{comment}



% \begin{figure*}[htb!]
% \centering
% \includegraphics[width=\textwidth]{figs/opt-plan-exp-5.jpg}
% \caption{(a) The cross-time plan space of a simple filter query,
% with target node $\{C\}$ and three time points $t_1\cdots t_3$.
% The arc between two arrows means``AND", it is a two-operand operation;
% otherwise, the relationship between arrows are ``OR" by default.
% (b) The execution time expanded cross-time plan space.
% Dotted arrows like $A_1\rightarrow A_1'$ means materialize table $A$ to disk,
% with cost $Save(A)$ contributing to the time at arrow's left side; $A_1'\rightarrow A_2'$ has zero cost;
% $A_1'\rightarrow A_2$ means load table from disk, with cost $Load(A)$.
% }
% \label{fig:opt-plan-exp-2}
% \end{figure*}

% To illustrate what cross-time planning means, the plan space of a simple query
% $Q = \sigma(R)$ is shown in Figure~\ref{fig:opt-plan-exp-2}(a).
% Assume data is continuously generated into the input table R and our goal is
% to generate the query result on R at time $t_3$ (node $C$).
% Now if we also want to consider two more time points $t_1$ and $t_2$ for potential progressive execution,
% and the input relation R can be accessed in either snapshot or delta form of $\Delta(t-1, t)$ at all three time points,
% then the arrows in Figure~\ref{fig:opt-plan-exp-2}(a) are all the valid TVR transformations defined by related rules.
% This is the plan space of the query considering time points $t_1\cdots t_3$.
% Every subtree in the directed graph rooted at $C$ with all leaf nodes below the dotted line is a valid plan.

% However, Figure~\ref{fig:opt-plan-exp-2}(a) is only "logical" plan in a sense that every arrow describes
% the operation and the data to operate on; arrow's execution time is not specified.
% In fact, different nodes and arrows in this graph can be executed at different sets of time points.
% For example, $A$ can be computed at $t_1, t_2$ or $t_3$, $B$ and $D$ can be only computed
% at $t_2$ or $t_3$ because their input data will not be available until $t_2$.

% Figure~\ref{fig:opt-plan-exp-2}(b) shows the execution time expanded \emph{cross-time plan} space,
% where the plan spaces of the three sub-plans at $t_1\cdots t_3$ are drawn within their own time ranges,
% incurring cost $c_1\cdots c_3$.
% In this figure, dotted arrows like $A_1\rightarrow A_1'$ means materialize table $A$ to disk,
% with cost $Save(A)$ contributing to the time at arrow's left side; $A_1'\rightarrow A_2'$ has zero cost;
% $A_1'\rightarrow A_2$ means load table from disk, with cost $Load(A)$.

% Figure~\ref{fig:opt-plan-exp-2}(b) depicts the full set of execution options in the cross-time plan space.
% For example, one plan is to run everything at $t_3$ in one shot,
% either via computing $B_3$ and $E_3$ first or compute $C_3$ directly from input data below.
% This execution at $t_3$ will take large of amount of resources and have a high latency.
% Another plan is ...., it spreads computation across time.
% Nevertheless the total amount of computation (and thus total resource consumption) is larger because of
% the progressive execution overhead (e.g. merging deltas into snapshots, writing/reading intermediate data to/from disk).
% Given the input data characteristics on R, the optimizer can estimate the cost of every arrow,
% sub-plan and thus the whole cross-time plan using existing cost estimation techniques,
% but which criteria should be used to compare plans and pick the optimal?


% Another related \botong{(not needed for now)} one is Property~\ref{prop:plan-composable} below,
% which is a stronger version of Property~\ref{prop:add}.
% (Property~\ref{prop:plan-composable} $\Rightarrow$ Property~\ref{prop:add})

% \begin{property} \label{prop:plan-composable}
% For any plan $P_1$ and $P_2$, we have $\mathbb{C}(P_1) + \mathbb{C}(P_2) = \mathbb{C}(P_1 + P_2)$,
% where $P_1 + P_2$ means running both plans together.
% \end{property}

% It is important to point out that during the DP, the cost of every arrow and node (that correspond to any time point $t_i$) should be
% calculated and compared in the terms of the score function $\mathbb{C}(c_1, \cdots, c_T)$ rather than $c_i$ itself.
% Changing score function $\mathbb{C}(P)$ will change the cost of every arrow, node, plan and thus the preferences over plans.

% For instance, the second score function (b) above $\mathbb{C}(P) = -\prod_{i = 1..T}{c_i(P)}$ does not satisfy Property~\ref{prop:add},
% and thus DP will not work for it.
% But DP does work for score functions (a) and (c).
% As a result, most traditional optimization techniques including volcano,
% sub-query/view materialization works can be applied directly under these score functions.

\begin{comment}
\noindent
\textbf{More Challenges}.
Many simplifying assumptions are made in the example to better visualize the cross-time plan space.
There are more challenges in the general optimization problem:

%Now we've shown how to extend the existing cost-based volcano framework to optimize a query instance and produce a TVR delta/snapshot plan.
%This opens up a large space of options for the scheduler and optimizer when we look across query instances. Specifically in this section, we tackled three problems.

%Now given the enhanced volcano optimizer that handles planning within each query instance, we need to tackle several problems when planning across the recurrent query instances.

\begin{enumerate}
\item Picking query(ies) and candidate execution time points ($t_1\cdots t_T$) to optimize for.
Cluster utilization, available data for various queries are all changing over time.
When and which query(ies) to optimize and thus potentially execute its sub-plan?
How to pick the set of time points to consider from the continuous time domain?
Intuitively, many aspects need to be considered, for example cluster utilization now and in the future,
the amount of potential benefit if executed at the moment (which depends on query structure,
the amount of new input data available so far, the amount that will arrive in the future and so on).

\item Nondeterministic future information, including query trigger time and order,
future input data characteristics (e.g. append-only or not, data distribution) and arrival rate.
When the optimizer is asked to produce a plan at the moment (say $t_1$ in the example),
it needs information about the future (at $t_2$ and $t_3$) in order to be able to cost and compare the overall plans,
so that the selected sub-plan is both efficient now and would benefit the future.
Without future information, what's optimal to run at $t_1$ alone might not be beneficial or even useful at all for later runs.
Obviously we cannot know the exact future, only estimations in terms of expectations or distributions can be provided.
How should volcano optimizer be improved to handle nondeterministic plan space?

\item Size of the search space. The search space for the query of a single filter operation is
already as complex in Figure~\ref{fig:opt-plan-exp-2}(b),
with only one incremental computing method and three execution time points.
In general, with a normal DAG of queries and many incremental computing methods combined,
multiplied by $T^2$ (\# of time points, expanded with execution time options),
the search space is huge and challenging.
How do we expand this space, and search for the best plan in it?
%DP is a popular choice in traditional volcano optimizer because of its efficiency and optimality guarantee.
%However, in our space, since the cost of every sub-plan appears independently in the final score function
%$\mathbb{C}(c_1(P), c_2(P), \cdots, c_s(P))$,
%DP's optimal substructure property might not hold across sub-plans in general.

\item Common sub-query sharing opportunities.
DP is a popular choice in traditional volcano optimizer because of its efficiency and optimality guarantee.
However it is well known that DP alone sacrifices the possibility to share results.
That's why works on multi-query optimizations and materialized view selection are developed on top of the basic DP over the years.
In our case, there are also lots of sharing opportunities,
across and within sub-plans at different time points, across and within target nodes.
To what extent can we re-use the works on common sub-query sharing?

%For example, Figure~\ref{fig:multi-target-exp} gives a plan space with two target nodes: $C$ and $D$.
%If planned independently with DP, we will choose $A\rightarrow C$ and $A\rightarrow D$ with total cost of eight.
%While if planned together, we can produce (and materialize) $B$ first, then do $B\rightarrow C$ and $B\rightarrow D$, with a total cost of six.
%In general, since DP assumes no sharing and thus always recompute in case of common nodes, it will not produce the optimal plan.

%Which intermediate node (e.g. delta/snapshot) at which run should we materialize for future use.
%When generating the plan of the current query instance, what (intermediate) node/data should we produce and save to enable more efficient plan for the next/all future run(s)?
%What we choose to save impacts the plan space of the next run, whose decision further impacts the plan space of the run after it. The search space seems to be exponential.

\end{enumerate}

%\begin{figure}[htb!]
%\centering
%\includegraphics[width=0.3\textwidth]{figs/multi-target-exp.jpg}
%\caption{Multi-target optimization}
%\label{fig:multi-target-exp}
%\end{figure}

Overall, this is an open problem because of the huge plan space as well as the nature of involved future unknowns.
There are also many research directions to explore, just to list a few: multi-query optimization,
sub-query/materialized view selection, dynamic planning, future planning, query scheduling, cluster-wide
resource scheduling across time, explore vs exploit of plans, uncertainty estimation, risk management and so on.
\end{comment}

% Under the settings of Section~\ref{sec:opt-def}, let us look closer to the optimization problem
% (described in Section~\ref{sec:opt-def}) assuming everything regarding all time points are known deterministically.

\subsection{Deciding States to Materialize}
\label{sec:mqo-sharing}

The problem of deciding the states to materialize
can be modeled as finding the sharing opportunities in the plan space.
% There are many sharing opportunities in the plan space,
% which can be crucial to the query performance.
In other words, a shared sub-plan between $P_i$ and $P_j$ in an incremental plan
is essentially an intermediate state that can be saved by $P_i$ and reused by $P_j$.
E.g., in Fig.~\ref{fig:temporal-space},
since both \op{HashInnerJoin} and \op{IncrHashInnerJoin} require shuffling $\s{S}{t_1}$ and $\s{R}{t_1}$,
the two relations can be shuffled only once and reused for both joins.
The parts \textcircled{1} and\textcircled{2} circled in dashed lines depict the sharable sub-plans.

Finding the optimal common sub-plans to share is a multi-query optimization (MQO) problem,
which has been extensively studied~\cite{mqo,mqo-jr,mqo-pods}.
% It is well known that DP alone sacrifices the possibility to share sub-plans,
% that's why works on multi-query optimizations and materialized view selection are developed on top of the basic DP over the years.
% The same problem exists here.
% For instance in Figure~\ref{fig:opt-plan-exp-2}(b), if in DP's optimal plan contains two paths
% (either for different targets nodes or for the same) that contains $A_1'$,
% it actually means computing $A_1$ twice and store it as $A_1'$ twice.
% Since our plan naturally includes saving tables to disk between time points, it further reduces the overhead of sharing:
% if $A_1$ is computed and saved as $A_1'$ already for one path,
% then sharing of $A_1'$ is almost free: we don't need to pay the extra saving cost.
% As a result, it is more favorable and beneficial for us to consider sharing of common nodes in the space.
In this work, we extend the latest MQO algorithm in~\cite{mqo-pods},
which proposes a greedy framework on top of Cascade-style optimizers for MQO.
% with various speed-up optimizations.
For the sake of completeness, we list the algorithm in
Algo.~\ref{alg:greedy}, by highlighting the extensions for progressive planning.
The algorithm runs in an iterative fashion.
In each iteration, it picks one more candidate from all possible shareable candidates,
which if materialized can minimize the plan cost (line 4),
where $bestPlan(\mathbb{S})$ means the best plan with $\mathbb{S}$ materialized and shared.
The algorithm terminates when all candidates are exhausted or adding candidates can no longer
improve the plan cost.
However, as incremental planning needs to consider the temporal dimension,
the shareable candidates are no longer solely the set of shareable sub-plans,
but pairs of a shareable sub-plan $s$ and a choice of its execution time $\et{s}$.
Pair $\langle s, \et{s} \rangle$ means computing and materializing the sub-plan $s$
at time $\et{s}$, which can only benefit the computation that happens after $\et{s}$.
For instance, considering the physical plan space in Fig.~\ref{fig:temporal-space},
the sharable candidates are $\{\langle \textcircled{1}, t_1 \rangle, \langle \textcircled{1}, t_2 \rangle, \langle \textcircled{2}, t_1 \rangle, \langle \textcircled{2}, t_2 \rangle\}$.
The speed-up optimizations in~\cite{mqo-pods} are still applicable to Algo.~\ref{alg:greedy}.

\begin{algorithm}[th]
\footnotesize
\algsetup{indent=2em}
\begin{algorithmic}[1]
\STATE $\mathbb{S}=\emptyset$
\STATE $\mathbb{C}=$ \textbf{shareable candidate set consiting of all shareable nodes and their potential execution times $\{\langle s, \et{s} \rangle\}$}
\WHILE {$\mathbb{C} \neq \emptyset$}
	\STATE Pick $\langle s, \et{s} \rangle \in \mathbb{C}$ that minimizes
  $\tilde{\mathfrak{c}}(bestPlan(\mathbb{S}'))$
  where $\mathbb{S}' = \{\langle s, \et{s} \rangle \} \cup \mathbb{S}$
	\IF {$\tilde{\mathfrak{c}}(bestPlan(\mathbb{S}')) < \tilde{\mathfrak{c}}(bestPlan(\mathbb{S}'))$}
		\STATE $\mathbb{C} = \mathbb{C} - \{\langle s, \et{s} \rangle\}$
    \STATE $\mathbb{S} = \mathbb{S}'$
	\ELSE
		\STATE $\mathbb{C}=\emptyset$
	\ENDIF
\ENDWHILE
\RETURN $\mathbb{S}$
\end{algorithmic}
\caption{Greedy Algorithm for MQO}
\label{alg:greedy}
\end{algorithm}

% Note that by running this algorithm once on the time expanded cross-time plan space of a DAG of queries,
% sharing opportunities between and within related queries, between and within sub-plans (time points) are all explored altogether.

As expanded with execution time options, the enumeration space of the shareable candidate set becomes much larger than the original algorithm in~\cite{mqo-pods}.
Interestingly, we find that under certain cost models we can reduce the enumeration space
down to a size comparable to the original algorithm, formally summarized in
Theorem~\ref{thm:store-early}.
Theorem~\ref{thm:store-early} relies on the fact that
materializing a shareable sub-plan at its earliest possible time
subsumes other materialization choices. Due to space limit, we omit the proof.

% Due to space limitation, we provide a proof sketch for the theorem.
%
%What we want to achieve is to be able to search through the space without having to expand the plan space with execution options (recall Figure~\ref{fig:opt-plan-exp-2}(a)vs(b)).
%
% \begin{property} \label{prop:time-computable}
% For any node $N$ in the cross-time plan space, if there is one way to compute $N$ at time $t$,
% then the whole subgraph rooted at $N$ are computable at time $t$.
% \end{property}
%
% \begin{property} \label{prop:prefer-early}
% For $\forall x_i, y \geq 0$, $1\leq i < j \leq T$:
% \[ \mathbb{C}(x_1, \cdots, x_T) \geq  \mathbb{C}(x_1, \cdots, x_i + y, \cdots, x_j - y, \cdots, x_T)\]
% \end{property}
\begin{theorem}
For cost function $\tilde{c}_w$ satisfying $w_i < w_j$ if $i < j$,
or cost function $\tilde{c}_v$ satisfying the property that
entry $i$ has a lower priority than entry $j$ if $i < j$ in the lexical order,
we only need to consider the earliest valid execution time for each shareable sub-plan.
That is, for each $s$, we only need to consider the shareable candidate $\langle s, min(\td{s}) \rangle$ in Algorithm~\ref{alg:greedy}.
% If Property~\ref{prop:time-computable} and~\ref{prop:prefer-early} hold,
% then for any node $N$ which can be computed at or after time point $t_n$,
% if we want to store $N$ into $N'$ at some point,
% then it is always better to (compute and) store it at time $t_n$, not any time later.
\label{thm:store-early}
\end{theorem}
% \begin{proof}
% Clearly materializing a shareable sub-plan at its earliest possible time
% subsumes other materialization choices, as any reuse opportunities can always choose
% between use or not use the materialized sub-plan.
% Therefore, the reuse cost of the shareable sub-plan does not increase.
% On the other hand, as the cost function strictly prefers an earlier execution time
% by assignment resources at an earlier time with a lower cost, the materialization overhead
% of the shareable sub-plan also does not increase.
% Combining the above two points, one can see the shareable candidate
% $\langle s, min(\td{s}) \rangle$ subsumes other candidates $\langle s, \cdot \rangle$.
% \end{proof}
% When Theorem~\ref{thm:store-early} holds,
% we can reduce the size of $R$ by a factor of $T$ (number of time points)
% and thus a much faster optimization process.

However, traditional ways of modeling physical operators
treat the inner implementation of operators as black boxes,
% which cannot describe the inner data structures used in the operators,
% and thus
which are not able to fully utilize the sharing opportunities.
To understand that, consider again \op{HashInnerJoin} and \op{IncrHashInnerJoin} in Fig.~\ref{fig:temporal-ex}.
Both joins build hash tables on one or multiple inputs.
By exploiting this, we can save not only the shuffling of the input data, but also the hash-building operations.
In \sys{}, we explicitly model all inner data structures of physical operators.
For instance, we model hash-based join operators by two separate operators \op{BuildHash} and \op{ProbeHash}.
\op{BuildHash} reads an input and builds a hash table in memory using the join predicates as keys.
\op{ProbeHash} reads the other input, probes the built hash table, and produces join tuples.
Fig.~\ref{fig:physical-plan} shows an example implementation of \op{HashInnerJoin} and \op{IncrHashInnerJoin}
using \op{BuildHash} and \op{ProbeHash}.
The \op{BuildHash} subtrees circled in dashed lines show another sharing opportunity.
Similar modeling can be applied to other operators such as hash-based aggregates.

\begin{comment}
\subsection{Plan search with nondeterministic future}
\label{sec:non-deterministic}

If the future is nondeterministic in a sense that there are multiple possible outcomes that
are very different from each other (as opposed to variations around an expected value),
the problem becomes more challenging.
For instance, in our setting with two time steps $t_1$ (now) and $t_2$ (future),
whether the future input data at $t_2$ is positive-only (does not contain retractions) can
lead to rather different execution options.

\begin{figure}[htb!]
\centering
\includegraphics[width=0.5\textwidth]{figs/non-deter-future.jpg}
\caption{The cross-time plan space of two possible outcomes at the future time step}
\label{fig:non-deter-future}
\end{figure}

Figure~\ref{fig:non-deter-future}(a) gives an example of the cross-time plan space with two possible outcomes at $t_2$.
Specifically, the cost of computing $B_2$ directly from input data can be either $100$ or $3$,
depending on whether the input data $t_2$ turns out to be positive-only.
Let's say we know the probability of each outcome,
how should we tackle this problem when the plan space itself is not deterministic?

It is natural to extend our optimization goal to minimize the expectation of the score function, i.e. $E(\mathbb{C}(P))$.
Along this thought, we can treat each possible outcome separately,
and conditional on one outcome the space is deterministic.
Figure~\ref{fig:non-deter-future}(b) shows the separated plan space with two possible outcome
$X$ and $Y$ separated from $B$.

It may seem that this problem can now be solve with techniques in Section~\ref{sec:deterministic}
because $X$ and $Y$ can be interpreted as two target nodes,
and we are looking for a plan that minimize a weighted sum of their costs.

However, a deeper thought reveals their fundamental discrepancies:
even though in the optimization target $E(\mathbb{C}(P))$,
$X$ and $Y$ appears to be weighted summed (implying an ``AND" logic),
but their actual relationship in the plan is a combination of ``AND" at $t_1$ and ``OR" at $t_2$.

Here is a quick explanation: consider the basic case of assuming no sharing,
and $P_X$ and $P_Y$ are the best plans for $X$ and $Y$ by DP respectively.
Let $P_X^1$ denote $P_X$'s sub-plan at $t_1$.
If $X$ and $Y$ are indeed two target nodes as in Section~\ref{sec:deterministic},
the cost of running $P_X + P_Y$ together would be
$\mathbb{C}(c(P_X^1 + P_Y^1), c(P_X^2 + P_Y^2))$.
If $X$ and $Y$ are two possible futures at $t_2$,
the expected cost of carrying out both plans together should be
%\begin{equation} \label{eqn:score-function}
$\mathbb{P}(X) \mathbb{C}\left( c(P_X^1 + P_Y^1), c(P_X^2) \right) + \mathbb{P}(Y) \mathbb{C}\left( c(P_X^1 + P_Y^1), c(P_Y^2) \right)$,
%\end{equation}
where $\mathbb{P}(X)$ and $\mathbb{P}(Y)$ denote the probability of $X$ or $Y$ actually happening.
Note that it is not $\mathbb{P}(X) \mathbb{C}\left( c(P_X^1), c(P_X^2) \right) + \mathbb{P}(Y) \mathbb{C}\left( c(P_Y^1), c(P_Y^2) \right)$ either.
In other words, at $t_1$, since we don't know which future ($X$ or $Y$) it will be, we need to run both $P_X^1$ and $P_Y^1$.
When we arrived $t_2$, we will know which future it is and thus only need to run that future's sub-plan at $t_2$.

This is similar to the concept of choose-plan operator described in~\cite{},
in the sense that the produced plan contains two possible sub-plans for $t_2$,
and only when we arrived at $t_2$ will we know which sub-plan we should run.

\noindent
\textbf{Search Strategy}. How should we search for the best plan in this setting?
To minimize the expectation $E(\mathbb{C}(P))$, would DP still work (produce the best plan)?
First, let's rewrite the optimization goal by defining a new score function $\mathbb{C}_{X,Y}$ using $\mathbb{C}$:
\begin{align*}
E(\mathbb{C}(P)) &= \mathbb{C}_{X,Y}(P^1, P_X^2, P_Y^2)\\
&=  \mathbb{P}(X) \mathbb{C}\left( c(P^1), c(P_X^2) \right) + \mathbb{P}(Y) \mathbb{C}\left( c(P^1), c(P_Y^2) \right)
\end{align*}
Where $P^1 = P_X^1 + P_Y^1$ is what's run at $t_1$.

\begin{theorem} \label{thm:dp-expectation}
If $\mathbb{C}$ satisfy Property~\ref{prop:add},
then $\mathbb{C}_{X,Y}$ as a new score function satisfies the property as well,
and according to Theorem~\ref{thm:dp}, DP also works for $\mathbb{C}_{X,Y}$.
\end{theorem}

With this, we can still use DP to produce the optimal $P_x$ and $P_y$ respectively, and that the combined plan
$(P_x^1 + P_y^1, P_X^2, P_Y^2)$ will have the smallest $\mathbb{C}_{X,Y}(P^1, P_X^2, P_Y^2)$ assuming no sharing.
Again, note that during the DP,
the cost of each arrow and node should be computed and compared in terms of $\mathbb{C}_{X,Y}(P^1, P_X^2, P_Y^2)$.
For instance, arrows at $t_1$ contributes to $P^1$. Arrows at $t_2$ contribute to either $P_X^2$ or $P_Y^2$,
which means when $\mathbb{P}(X) \neq \mathbb{P}(Y)$, the cost (expressed in terms of $\mathbb{C}_{X,Y}(P^1, P_X^2, P_Y^2)$)
of the same arrow at $t_2$ will appear different when we are DPing for $X$ versus $Y$.

For instance in Figure~\ref{fig:non-deter-future}(b), assume $\mathbb{P}(X) = 0.75, \mathbb{P}(Y) = 0.25$,
and $\mathbb{C}(c_1, c_2) = 0.5 c_1 + c_2$ (that's why cost of $C\rightarrow A_1$ is a half of $D\rightarrow A_2$).
By running DP without sharing, we get $P_X^1 = C \rightarrow A_1 \rightarrow A_1', P_X^2 = A_1' \rightarrow A_2 \rightarrow X$,
and $P_Y^1 = \varnothing, P_Y^2 = E \rightarrow Y$. Combining the plans give us
$E(\mathbb{C}(P)) = \mathbb{C}_{X,Y}(P^1, P_X^2, P_Y^2) = 0.75(4 + 1) + 0.25(4 + 3) = 5.5$.

\noindent
\textbf{Consider Sharing}.
As discussed in Section~\ref{sec:deterministic}, consider sharing on top of basic DP can open up more opportunities.
Again we can use Algorithm~\ref{alg:greedy} (modified) to greedily compute the set of nodes to share,
by replacing $\mathbb{C}(bestPlan(S))$ with $\mathbb{C}_{X, Y}(bestPlan(S))$.

In the above example, if we save and share $A_1$ at $t_1$, doing $A_1' \rightarrow A_2 \rightarrow X$ or $Y$ at $t_2$
is a better plan with $E(\mathbb{C}(P)) = 0.75(4 + 1) + 0.25(4 + 1) = 5$.

On the other hand, if $Y$ is more likely to happen than $X$, say $\mathbb{P}(X) = 0.25, \mathbb{P}(Y) = 0.75$,
the best plan changes.
Firstly, the basic DP plan with no sharing changes for $X$:
it will choose $D\rightarrow A_2$ over $C \rightarrow A_1 \rightarrow A_1' \rightarrow A_2$
because $0.25\times 4 + 0.75\times 4 > 0.25 \times 8$.
So that the base plan with no sharing has $E(\mathbb{C}(P)) = 0.25(0 + 9) + 0.75(0 + 3) = 4.5$.
When the cost of sharing $A_1$ still turns out to be $E(\mathbb{C}(P)) = 0.25(4 + 1) + 0.75(4 + 1) = 5$,
Algorithm~\ref{alg:greedy} will terminate returning the base plan with no sharing:
$P^1 = \varnothing, P_X^2 = D\rightarrow A_2 \rightarrow X, P_Y^2 = E\rightarrow Y$.


\noindent
\textbf{More on Sharing}. Now let's dive deeper into details in Algorithm~\ref{alg:greedy}.
The first thing is that Theorem~\ref{thm:store-early} no longer hold here.
The reason is that the same amount of work (computing and saving a node) at $t_1$ and $t_2$ have
different probability weights when contributing into $\mathbb{C}_{X,Y}(P^1, P_X^2, P_Y^2)$.
As a result, both $A_1$ and $A_2$ should be in the candidate set $R$ regardless.
Furthermore, for candidates at $t_2$, the best choice can be sharing
in the case of $X$ (in $P_X^2$), but not in the case of $Y$ (not in $P_Y^2$).
In other words, the choice of sharing itself might be conditional on which future turns out.

Formally, we define a future state set $F_i$ for every time point $t_i$,
which contains all the possible future states in $t_i$.
In this example, $F_2 = \{X, Y\}$ and $F_1 = \{\#\}$, where $\#$ stands for the sole possible state at $t_1$.
Next, each $s\in S$ in Algorithm~\ref{alg:greedy} becomes a pair $\langle N_i, V_i \rangle$.
It means to save and share node $N_i$ at $t_i$ only for the set of future states in $V_i$,
where $V_i \subseteq F_i$ is called the validity set of the shared node $N_i$.
For instance, the validity set of $A_1$ can be $\varnothing$ (do not share) or $\{\#\}$ (always share).
The validity set of $A_2$ can be $\varnothing$, $\{X\}$, $\{Y\}$, or $\{X,Y\}$.

Finally, we give the updated version of Algorithm~\ref{alg:greedy} in Algorithm~\ref{alg:greedy-non-deter},
where again $bestPlan(S)$ means the plan produced by DP that generates all target nodes assuming
nodes in $S$ is saved and shared in their corresponding validity sets.
In each round of the greedy process, we determine the validity set of each candidate also greedily.

\begin{algorithm}[th]
\caption{Updated version of Algorithm~\ref{alg:greedy}, under the nondeterministic future case}
\label{alg:greedy-non-deter}
\algsetup{indent=2em}
\begin{algorithmic}[1]

\STATE $S=\varnothing$
\STATE $R=$ all nodes in the plan space (candidate set)
\WHILE {$R\neq \varnothing$}
  \STATE $s = \varnothing$
  \FOR {$N_i\in R$}
    \STATE $V_i = \varnothing$ (validity set)
    \FOR {$v \in F_i$}
      \STATE Add $v$ into $V_i$ if it reduces $\mathbb{C}_{X, Y}(bestPlan(\{\langle N_i, V_i \rangle \} \cup S))$
    \ENDFOR
    \STATE Replace $s$ with $\langle N_i, V_i \rangle$ if it reduces $\mathbb{C}_{X, Y}(bestPlan(\{s\}\cup S))$
  \ENDFOR

  \IF {$\mathbb{C}_{X, Y}(bestPlan(\{s\}\cup S)) < \mathbb{C}_{X, Y}(bestPlan(S))$}
    \STATE $R = R - \{s.field1\}; S = S\cup \{s\}$
  \ELSE
    \RETURN $S$
  \ENDIF
\ENDWHILE
\RETURN $S$

\end{algorithmic}
\end{algorithm}
\end{comment}

%Next we zoom into the optimizer and discuss in detail under two scenarios: recurrent queries (multiple instances of the same query ran on different chunks of data over time) and query pipeline (DAG of queries).

%\subsection{Planning Recurrent Queries}

%Assuming continuous data ingestion, the same query is ran multiple times, each instance is ran on different chunks of input data over time. Consider the following two use cases.

%\begin{enumerate}
%\item We need a daily summary over data arrived within the last 24h everyday. Traditionally we have to wait until 0AM when all data becomes available and then kickoff the query to compute the summary. This is typically a big batch job that takes lots of resource (machine hour), has a big resource footprint (parallelism), and has a big latency.

%In fact, in \company{} we have lots of ``baseline queries'' to run at midnight everyday. They are pipelines of analytical queries that produce critical operational data and business insights for various teams and services. From our (data warehouse's) perspective, this is a group of large and high priority batch queries submitted around the same time everyday. They typically occupy our entire cluster for a very long time, and other low priority jobs has to queue up and wait.

%With progressive computation framework, it is now possible for us to run these baseline queries incrementally over time, similar to the mini-batch in Spark Streaming \cite{}. For example we can trigger one query instance every three hours, which generates a TVR delta for the pass three hours' worth of data. At the end of the day, we only need to merge the eight deltas into a final TVR snapshot.

%There are two major benefits here:
%\begin{itemize}
%\item Smoothing cluster resource usage over time. More importantly, the system can decide when to trigger the query instances and shape the resource usages over time, without any query modification and user intervention.

%\item Much smaller query latency for the final run triggered at 0AM at the end of the day. Moving batch towards streaming style of execution, we are getting the streaming benefits.
%\end{itemize}


%\item Repetitive computation. We also have a slightly different use case. Rather than once per day, the user requests four summaries per day, at 6AM, 12PM, 6PM and 0AM respectively. Specifically, the run at 6PM takes the data arrived between 0AM-6PM that day as input. Apparently these runs have lots of computation overlap, the later runs always include the computation of the early ones.

%With the TVR model, we can easily avoid the redundant computation without having to ask the user to rewrite their query pipeline. Instead of producing the snapshot from scratch, each run only computes a delta over the new data since last run and merge with the previous snapshot to produce the current snapshot.
%\end{enumerate}

%Thoughts: look only one step forward. Assume there will be only one final run after the current run. Choose a plan that minimize the total cost of both runs. (Need to estimate future input data as well? )

%\subsection{Planning Query Pipeline}

%For a pipeline/DAG of queries, each query can be triggered at different time points. Other than the two points in the previous subsection, we also need to decide the output format (delta/snapshot/both?) of each query instance, because the output of a query might be consumed by more than one downstream queries, each might have different preferences over input data format.


==> motivation.tex <==
%!TEX root=main.tex

\section{Motivation}
Cluster analysis:
\begin{itemize}
    \item cluster usage pattern
    \item pipeline complexity: deep pipeline, hard deadline
\end{itemize}
- resource periodic usage pattern in a long time (e.g., month): cpu, memory/IO, storage

- baseline dependency depth: ETL followed by analysis
    - with or without aggregation
    - how many dependent downstream queries


We should draw the following figures:
\begin{enumerate}
    \item CDF of (\# of dependent downstream queries) in baselines
    \item CDF of (depth of baselines), also mentioning (not necessarily with figures) that the general pattern of baselines is ETL followed by analysis, and thus early output can enable early execution of downstream queries
    \item total CPU hours spent per level of baselines (level in the baseline dependency graph)
    \item input data cumulation rate of all baseline jobs over the day
    \item CPU usage curve across a day
\end{enumerate}

NOTE: workloads from different applications. Maybe similar analysis on non-\company{} workloads?

